Deep Anomaly Detection under Labeling Budget Constraints

Selecting informative data points for expert feedback can significantly improve the performance of anomaly detection (AD) in various contexts, such as medical diagnostics or fraud detection. In this paper, we determine a set of theoretical conditions under which anomaly scores generalize from labeled queries to unlabeled data. Motivated by these results, we propose a data labeling strategy with optimal data coverage under labeling budget constraints. In addition, we propose a new learning framework for semi-supervised AD. Extensive experiments on image, tabular, and video data sets show that our approach results in state-of-the-art semi-supervised AD performance under labeling budget constraints.

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/ablation-weight.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/cifar_query_weight.pdf}
    \includegraphics[width=0.45\linewidth]{images/fmnist_query_weight.pdf}
    \caption{Ablation study on the weighting scheme in \Cref{eqn:loss-2}. With different query budgets $|\gQ|$, the performance on image datasets degrades both upon down-weighting (0.01, 0.1) or up-weighting (10.0) the queried samples. In contrast, equal weighting yields optimal results. } 
    \label{fig:ablation-weight}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/ablation_query.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{images/query_comp_new_legend.pdf}
    \caption{Ablation study on the query strategy. K-Means++ significantly outperforms other strategies for active anomaly detection on most of the datasets.} 
    \label{fig:ablation-query}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/ablation_true_est_ratio.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{images/true_est_ratio_comp_new_legend.pdf}
    \vspace{-10pt}
    \caption{Model using the estimated ratio is indistinguishable from the one using the true ratio.} 
    \label{fig:ablation-true-est-ratio}
\end{figure}



==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/corr_mat.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\linewidth]{images/corr_mat_cifar10_0.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_cifar10_1.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_fmnist_0.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_fmnist_1.pdf}
    \caption{Anomaly score correlation matrix $\langle S(\vx_i),S(\vx_j)\rangle$, where $\vx_i$ and $\vx_j$ are jointly sampled in the same query set. The result indicates that anomaly scores can be considered as approximately independent random variables.
    } 
    \label{fig:corr-mat}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/grad-diverse-comparison.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/grad_diverse_compare_cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/grad_diverse_compare_fmnist.pdf}
    \caption{Comparison with gradient diversity querying strategy (BADGE)~\citep{ash2020deep}. The gradients wrt. the penultimate layer representation don't provide as informative queries as the representation itself, thus outperformed by our querying strategy \gls{aloe}. The true contamination ratio is 10\%.} 
    \label{fig:grad-div-comparison}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/image_benchmark.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.85\linewidth]{images/error_years.png}
  \caption{Error (in $\%$ of 1-AUCROC) of ten methods on CIFAR10: two shallow methods (SVDD \citep{TaxD04} and IF \citep{liu2008isolation}) and eight deep methods (VAE \citep{kingma2014vae}, DCAE \citep{makhzani2015winner}, ADGAN \citep{deecke2018image}, DSVDD \citep{ruff2018deep}, GT \citep{golan2018deep}, MHRot \citep{hendrycks2019using}, Contrastive \citep{sohn2020learning}, and NTL \citep{qiu2022latent}). \gls{ntl} achieves the best anomaly detection performance on CIFAR10.
    \label{fig:image_benchmark}}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/image_data.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/img_res_font+_new_legend.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs the best among the compared methods on all query budgets.}
    \label{fig:img_data}
\vspace{-10pt}
\end{figure*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/image_data_batch_seq.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{images/img_res_seq.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs better than a sequential version.}
    \label{fig:img-data-seq}
\vspace{-10pt}
\end{figure*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/image_data_comparison_bce.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{images/img_res_bce.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. Deep \gls{ad} model (\gls{ntl}) performs significantly better than a binary classifier.}
    \label{fig:img-data-bce}
\vspace{-10pt}
\end{figure*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/robust-ratio.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.01.pdf}
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.05.pdf}
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.2.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets and data contamination ratios (1\%-top row, 5\%-middle row, 20\%-bottom row). Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs the best on all three contamination ratio setups.}
    \label{fig:robust-ratio}
\vspace{-10pt}
\end{figure*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/semisuper-comparison.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/semisuper_compare_cifar10_new_legend.pdf}
    \includegraphics[width=0.45\linewidth]{images/semisuper_compare_fmnist_new_legend.pdf}
    \caption{Comparison with semi-supervised learning fraemworks, FixMatch \citep{sohn2020fixmatch}, $k$-nearest neighbors \citep{iscen2019label}, and Gaussian process \citep{li2018pseudo}. On F-MNIST, \gls{aloe} outperforms all baselines, while on CIFAR-10, \gls{aloe} has a comparable performance with FixMatch with \kmeans querying.} 
    \label{fig:semisuper-comparison}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/thm1-delta.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/thm1_check_delta_cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/thm1_check_delta_fmnist.pdf}
    \caption{Cover radius $\delta$ (\Cref{eq:delta-est}) resulted from different querying strategies on the first class of CIFAR-10 and F-MNIST. Diverse queries systematically have smaller cover radius than other querying strategies.} 
    \label{fig:thm1-delta}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/thm1-ranking.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/rank-unlabeled-cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/rank-unlabeled-fmnist.pdf}
    \caption{Ranking performance of unlabeled data. AUC of unqueried data is evaluated using the fitted anomaly detector on the queried data. Our proposed diverse querying (\kmeans) provides better ranking of the unlabeled data.} 
    \label{fig:ranking-unquery}
\end{figure}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/toy_example.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/toy_example_fewer_query_new_order_v2.pdf}
    \vspace{-10pt}
    \caption{Anomaly score contour plots on 2D toy data demonstrate that \gls{aloe} [ours, (\textbf{d})] with only one labeled sample can achieve detection accuracy that is competitive with a fully supervised approach (\textbf{a}). Binary classification (\textbf{b}) is problematic for \gls{ad} since it cannot detect new anomalies, e.g. in the upper right corner of the plot. Subplot (\textbf{c}) demonstrates that unsupervised \gls{ad} is challenging with contaminated data. Even a single labeled query, in combination with our approach, can significantly improve \gls{ad}.}
    
    \label{fig:toy-data}
\vspace{-10pt}
\end{figure*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/figures/video_data.tex <==
\begin{figure}[ht]
\vspace{-10pt}
    \centering
    \includegraphics[width=0.85\linewidth]{images/video_res_c3e-1_font+_new_legend_wide.pdf}
\vspace{-10pt}
    \caption{Results on the video dataset UCSD Peds1 with different query budgets. \gls{aloe} achieves the leading performance.
    } 
    \label{fig:video_data}
 \vspace{-10pt}
\end{figure}



==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/header.tex <==
\PassOptionsToPackage{numbers, sort&compress}{natbib}

\usepackage[accepted]{icml2023}



\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage[hidelinks]{hyperref}  
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %
\usepackage{multirow}
\usepackage[pdftex]{graphicx}
\usepackage{dsfont}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{float}
\bibliographystyle{unsrtnat}


\usepackage{xr-hyper}
\newcommand{\theHalgorithm}{\arabic{algorithm}}

\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}


\usepackage{glossaries-extra}
\setabbreviationstyle[acronym]{long-short}
\glssetcategoryattribute{acronym}{nohyperfirst}{true}
\renewcommand*{\glsdonohyperlink}[2]{%
 {\glsxtrprotectlinks \glsdohypertarget{#1}{#2}}}
\usepackage{xfrac}
\input{math-commands}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\def\Ln{L_0^\theta}
\def\La{L_1^\theta}
\def\Ia{y}
\def\I{\mathds{1}}
\newacronym{loe}{LOE}{latent outlier exposure}
\newacronym{aloe}{SOEL}{\textbf{s}emi-supervised \textbf{o}utlier \textbf{e}xposure with a \textbf{l}imited labeling budget}
\newacronym{ntl}{NTL}{neural transformation learning}
\newacronym{mhrot}{MHRot}{multi-head RotNet}
\newacronym{ad}{AD}{anomaly detection}

\def\s{S}
\def\sau{s_1}%
\def\snu{s_0}%
\def\saq{\mu_1}%
\def\snq{\mu_0}%
\def\fz{f_z}
\def\unif{\text{Unif}}
\def\kmeans{k-means++ }
\newcommand{\ditto}[1][.4pt]{superv. (\Cref{eqn:loss})}
\def\Margin{\text{Mar}}
\def\HybridA{\text{Hybr1}}
\def\PositiveB{\text{Pos1}}
\def\PositiveA{\text{Pos2}}
\def\RandomA{\text{Rand1}}
\def\RandomB{\text{Rand2}}
\def\HybridB{\text{Hybr2}}
\def\HybridC{\text{Hybr3}}
\Crefname{figure}{Fig.}{Figs.}
\Crefname{table}{Tab.}{Tabs.}
\Crefname{section}{Sec.}{Secs.}
\Crefname{proposition}{Prop.}{Props.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{appendix}{Supp.}{Supps.}
\Crefname{theorem}{Thm.}{Thms.}
\Crefname{algorithm}{Alg.}{Algs.}

\newcommand{\sm}[1]{{\color{blue} \bf SM: #1}}
\newcommand{\mrr}[1]{{\color{green} \bf MR: #1}}


\usepackage{booktabs,array}
\def\Midrule{\midrule[\heavyrulewidth]}
\newcount\rowc

\def\ttabular{%
\hbox\bgroup
\let\\\cr
\def\rulea{\ifnum\rowc=\@ne \hrule height 1.3pt \fi}
\def\ruleb{
\ifnum\rowc=1\hrule height 1.3pt \else
\ifnum\rowc=6\hrule height \heavyrulewidth 
   \else \hrule height \lightrulewidth\fi\fi}
\valign\bgroup
\global\rowc\@ne
\rulea
\hbox to 10em{\strut \hfill##\hfill}%
\ruleb
&&%
\global\advance\rowc\@ne
\hbox to 10em{\strut\hfill##\hfill}%
\ruleb
\cr}
\def\endttabular{%
\crcr\egroup\egroup}


\newcommand{\al}[1]{{\color{blue} #1}}
\newcommand{\rbt}[1]{#1}





==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/math-commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\erf}{\mathrm{\,erf}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/abstract.tex <==
\begin{abstract}
Selecting informative data points for expert feedback can significantly improve the performance of \gls{ad} in various contexts, such as medical diagnostics or fraud detection. In this paper, we determine a set of theoretical conditions under which anomaly scores generalize from labeled queries to unlabeled data. Motivated by these results, we propose a data labeling strategy with optimal data coverage under labeling budget constraints. In addition, we propose a new learning framework for semi-supervised \gls{ad}. 
Extensive experiments on image, tabular, and video data sets show that our approach results in state-of-the-art semi-supervised \gls{ad} performance under labeling budget constraints.
\end{abstract}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/acknowledgement.tex <==
\section*{Acknowledgements}
SM acknowledges support by the National Science Foundation (NSF) under an NSF CAREER Award, award numbers 2003237 and 2007719, by the Department of Energy under grant DE-SC0022331, by the HPI Research Center in Machine Learning and Data Science at UC Irvine, by the IARPA WRIVA program, and by gifts from Qualcomm and Disney. Part of this work was conducted within the DFG research unit FOR 5359 on Deep Learning on Sparse Chemical Process Data. MK acknowledges support by the Carl-Zeiss Foundation, the DFG awards KL 2698/2-1, KL 2698/5-1, KL 2698/6-1, and KL 2698/7-1, and the BMBF awards 03|B0770E and 01|S21010C.

The Bosch Group is carbon neutral. Administration, manufacturing and research activities do no longer leave a carbon footprint. This also includes GPU clusters on which the experiments have been performed.

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:discussion}




We introduced semi-supervised outlier exposure with a limited labeling budget (\gls{aloe}). 
Inspired by a set of conditions that guarantee the generalization of anomaly score rankings from queried to unqueried data, we proposed to use a diversified querying strategy %
and a combination of two losses for queried and unqueried samples. By weighting the losses equally to each other and by estimating the unknown contamination rate from queried samples, we were able to make our approach free of its most important hyperparameters, making it easy to use. An extensive empirical study on images, tabular data, and video 
confirmed the efficacy of \gls{aloe} as a semi-supervised learning framework compatible with many existing losses for \gls{ad}.


\textbf{Limitations:} The success of our approach relies on several heuristics that we demonstrated were empirically effective but that cannot be proven rigorously. Estimation of the contamination ratio can be noisy when the query set is small---but the LOE loss is robust even under misspecification of the contamination ratio \citep{qiu2022latent}. The diversified sampling strategy becomes expensive when the dataset is large, but this can be mitigated by random data thinning.%

\textbf{Societal Impacts:} The use of human labels for anomaly detection runs the risk of introducing potential human biases in the definition of what is anomalous, particularly for datasets involving human subjects. Since our approach relies heavily on a relatively small number of human labels, the deployment of our approach with real human labelers would benefit by having guidelines for the labelers in terms of providing fair labels and avoiding amplification of bias.

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\input{tables/methods}
We study \gls{aloe} on standard image benchmarks, medical images, tabular data, and surveillance videos.
Our extensive empirical study establishes how our proposed method compares to eight \gls{ad} methods with labeling budgets implemented as baselines.
We first describe the baselines and their implementations (\Cref{tab:baselines}) and then the experiments on images (\Cref{sec:image_exp}), tabular data (\Cref{sec:tab_exp}), videos (\Cref{sec:video_exp}) and finally additional experiments (\Cref{sec:add-exp}). %

\input{tables/results}
\textbf{Baselines.} 
Most existing baselines apply their proposed querying and training strategies to shallow \gls{ad} methods or sub-optimal deep models (e.g., autoencoders \citep{zhou2017anomaly}).
In recent years, these approaches have consistently been outperformed by self-supervised \gls{ad} methods \citep{hendrycks2019using}. For a fair comparison, we endow all baselines with the same self-supervised backbone models also used in our method. %
By default we use \gls{ntl} \citep{qiu2021neural} as the backbone model, which was identified as state-of-the-art in a recent independent comparison of 13 models \citep{alvarez2022revealing}. Results with other backbone models are shown in \Cref{app:ablation_model}. %

The baselines are summarized in \Cref{tab:baselines} and detailed in \Cref{sec:baselines}.  
They differ in their querying strategies (col. 3) and training strategies (col. 4 \& 5): the unlabeled data is either ignored or modeled with a one-class objective. 
Most baselines incorporate the labeled data by a supervised loss (\Cref{eqn:loss}).
As an exception, \citet{ning2022deep} remove all queried anomalies and then train a weighted one-class objective on the remaining data. All baselines weigh the unsupervised and supervised losses equally. 
They differ in their querying strategies, summarized below:
\vspace{-7pt}
\begin{itemize}[leftmargin=*,itemsep=-2pt]
    \item {\bf Margin query} selects samples close to the boundary of the normality region deterministically. The method uses the true contamination ratio to choose an ideal boundary.
    \item {\bf Margin diverse query} combines margin query with neighborhood-based diversification. 
    It selects samples that are not $k$-nearest neighbors of the queried set.
    Thus samples are both diverse and close to the boundary.
    \item {\bf Most positive query} always selects the top-ranked samples ordered by their anomaly scores.
    \item {\bf Positive diverse query} combines querying according to anomaly scores with distance-based diversification. 
    The selection criterion combines anomaly score and the minimum Euclidean distance to all queried samples.
    \item {\bf Random query} draws samples uniformly.  
    \item {\bf Positive random query} samples uniformly among the top $50\%$ data ranked by anomaly scores.  
\end{itemize}
\vspace{-2pt}

\textbf{Implementation Details.}
In all experiments, we use a \gls{ntl} \citep{qiu2021neural} backbone model for all methods.  %
Experiments with other backbone models are shown in \Cref{app:ablation_model}.
On images and videos, \gls{ntl} is built upon the penultimate layer output of a frozen ResNet-152 pre-trained on ImageNet.
\gls{ntl} is trained for one epoch, after which all $|\gQ|$ queries are labeled at once. %
The contamination ratio $\alpha$ in \gls{aloe} is estimated immediately after the querying step and then fixed for the remaining training process. 
We follow \citet{qiu2022latent} and set $\tilde{y}_i = 0.5$ for inferred anomalies. This accounts for the uncertainty of whether the sample truly is an anomaly. More details are given in \Cref{sec:implementation} and \Cref{alg:aloe}.


\input{figures/image_data}
\subsection{Experiments on Image Data}
\label{sec:image_exp}
We study \gls{aloe} on standard image benchmarks to establish how it compares to eight well-known baselines with various querying and training strategies.
Informative querying plays an important role in medical domains where expert labeling is expensive. Hence, we also study nine medical datasets from \citet{medmnistv2}. 
We describe the datasets, the evaluation protocol, and finally the results of our study.


\textbf{Image Benchmarks.}
We experiment with two popular image benchmarks: CIFAR-10 and Fashion-MNIST. These have been widely used in previous papers on %
deep \gls{ad}  
\citep{ruff2018deep,golan2018deep,hendrycks2019using,bergman2020classification}. 


\textbf{Medical Images.}
Since medical imaging is an important practical application of \gls{ad}, we also study \gls{aloe} on medical images. The datasets we consider cover different data modalities (e.g., X-ray, CT, electron microscope) and their characteristic image features can be very different from natural images.   
Our empirical study includes all 2D image datasets presented in \citet{medmnistv2}
that have more than 500 samples in each class, including \rbt{Blood, OrganA, OrganC, OrganS, OCT, Pathology, Pneumonia, and Tissue.} 
We also include \rbt{Dermatoscope} but restricted to the classes with more than 500 training samples. %

\textbf{Evaluation Protocol.}
We follow the community standard known as the ``one-vs.-rest'' protocol to turn these classification datasets into a test-bed for \gls{ad} \citep{ruff2018deep,hendrycks2019using,bergman2020classification}.
While respecting the original train and test split of these datasets, the protocol iterates over the classes and treats each class in turn as normal. Random samples from the other classes are used to contaminate the data. The training set is then a mixture of unlabeled normal and abnormal samples with a contamination ratio of $10\%$ \citep{ruff2019deep,wang2019effective,qiu2022latent}. 
This protocol can simulate a ``human expert'' to provide labels for the queried samples because the datasets provide ground-truth class labels.
The reported results (in terms of AUC $\%$) for each dataset are averaged over the number of experiments (i.e., classes) and over five independent runs. %



 

\textbf{Results.}
We report the evaluation results of our method (\gls{aloe}) and the eight baselines on all eleven image datasets in \Cref{tab:img_results}. 
When querying 20 samples, our proposed method \gls{aloe} significantly outperforms the best-performing baseline by 6 percentage points on average across all datasets.
We also study detection performance as the query budget increases from $20$ to $160$ in \Cref{fig:img_data}. %
The results show that, with a small budget of 20 samples, \gls{aloe} (by querying diverse and informative samples) makes better usage of the labels than the other baselines and thus leads to better performance by a large margin. As more samples are queried, the performance of almost all methods increases but even for $160$ queries when the added benefit from adding more queries starts to saturate, \gls{aloe}  still outperforms the baselines.
\vspace{-0.5em}

\input{tables/tabular}
\subsection{Experiments on Tabular Data}
\label{sec:tab_exp}
Many practical use cases of \gls{ad} (e.g., in health care or cyber security) are concerned with tabular data.
For this reason, we study \gls{aloe} on four tabular datasets from various domains. We find that it outperforms existing baselines, even with as few as 10 queries. We also confirmed the fact that our deep models are competitive with classical methods for tabular data in \Cref{app:more-comp}.

\textbf{Tabular Datasets.} 
Our study includes the four multi-dimensional tabular datasets from the ODDS repository which have an outlier ratio of at least $30\%$. This is necessary to ensure that there are enough anomalies available to remove from the test set and add to the clean training set (which is randomly sub-sampled to half its size) to achieve a contamination ratio of $10\%$. The datasets are BreastW, Ionosphere, Pima, and Satellite. %
As in the image experiments, there is one round of querying, in which $10$ samples are labeled. For each dataset, we report the averaged F1-score (\%) with standard deviations over five runs with random train-test splits and random initialization. %

\textbf{Results.}
\gls{aloe} performs best on 3 of 4 datasets and outperforms all baselines by 3.2 percentage points on average. Diverse querying best utilizes the query budget to label the diverse and informative data points, yielding a consistent improvement over existing baselines on tabular data. 


\subsection{Experiments on Video Data}
\label{sec:video_exp}
\input{figures/video_data}

Detecting unusual objects in surveillance videos is an important application area for \gls{ad}. Due to the large variability in abnormal objects and suspicious behavior in surveillance videos, expert feedback is very valuable to train an anomaly detector in a semi-supervised manner. We use \gls{ntl} as the backbone model and  study \gls{aloe} on a public surveillance video dataset (UCSD Peds1). The goal is to detect abnormal video frames that contain non-pedestrian objects. %

Following \citet{pang2020self}, we subsample a mix of normal and abnormal frames for training (using an anomaly ratio of $0.3$) and use the remaining frames for testing.
Before running any of the methods, a ResNet pretrained on ImageNet is used to obtain a fixed feature vector for each frame. We vary the query budget from $|\gQ|=20$ to $|\gQ|=160$ and compare \gls{aloe} to all baselines. %
Results in terms of average AUC and standard error over five independent runs are reported in \Cref{fig:video_data}. \gls{aloe} consistently outperforms all baselines, especially for smaller querying budgets. %



\subsection{Additional Experiments}
\label{sec:add-exp}
In \Cref{app:ablation}, we provide additional experiments and ablations demonstrating \gls{aloe}'s strong performance and justifying modeling choices. The three most important findings are:
\vspace{-8pt}
\begin{itemize}[leftmargin=*,itemsep=-4pt]
\item {\bf \gls{aloe} vs. Active Learning:} Our framework is superior to its extension to the sequential active learning (\Cref{fig:img-data-seq}).
\item {\bf Varying Contamination Ratio:} \Cref{fig:robust-ratio} demonstrates that \gls{aloe} dominates under varying contamination ratios (1\%, 5\%, 20\%). In addition, \Cref{tab:alpha-estimate} confirms that \Cref{eq:alpha-is} reliably estimates 
 $\alpha$ on both CIFAR-10 and F-MNIST. 
\item {\bf Backbone Models:} \Cref{tab:backbone-dsvdd-mhrot} 
shows that \gls{aloe} also performs best for the backbone models  MHRot~\citep{hendrycks2019using} and DSVDD~\citep{ruff2018deep}.
\end{itemize}
\vspace{-8pt}
In addition, we provide an ablation of the temperature $\tau$ (\Cref{tab:ablation-tau}), a discussion on the effects of initialization randomness (\Cref{app:rand-init}), an ablation study of the pseudo-label $\tilde y$ values (\Cref{tab:ablation-pseudo-y}), a comparison to binary classification (\Cref{fig:img-data-bce}), an ablation of the \gls{aloe} loss components, an ablation of querying strategies (\Cref{fig:ablation-query}),
additional methods for inferring $y$  (\Cref{fig:semisuper-comparison}), and comparison to additional semi-supervised baselines (\Cref{fig:semisuper-comparison}, \Cref{tab:tab_knn}).





==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/introduction.tex <==
\section{Introduction}
Detecting anomalies in data is a fundamental task in machine learning with applications across multiple domains, from industrial fault detection to medical diagnosis. The main idea is to train a model (such as a neural network) on a data set of ``normal'' samples to minimize the loss of an auxiliary (e.g., self-supervised) task. Using the loss function to score test data, one hopes to obtain low scores for normal data and high scores for anomalies \citep{ruff2021unifying}. 

In practice, the training data is often contaminated with unlabeled anomalies that differ in unknown ways from the i.i.d. samples of normal data. 
No access to a binary anomaly label (indicating whether a sample is normal or not) makes learning the anomaly scoring function from contaminated data challenging; the training signal has to come exclusively from the input features (typically real-valued vectors).  Many approaches either assume that the unlabeled anomalies are too rarely encountered during training to affect learning \citep{wang2019effective} or try to detect and exploit the anomalies in the training data (e.g., \citet{qiu2022latent}).

While \gls{ad} is typically an unsupervised training task, sometimes expert feedback is available to check if individual samples are normal or not. For example, in a medical setting, one may ask a medical doctor to confirm whether a given image reflects normal or abnormal cellular tissue. Other application areas include detecting network intrusions or machine failures. Anomaly labels are usually expensive to obtain but are very valuable to guide an anomaly detector during training. For example, in \Cref{fig:toy-data}, we can see that our method, with only one labeled query (\Cref{fig:toy-data}~d) is almost on par with supervised \gls{ad} (\Cref{fig:toy-data}~a). However, the supervised setting is unrealistic, since expert feedback is typically expensive. Instead, it is essential to develop effective strategies for querying informative data points. 


Previous work on \gls{ad} under a labeling budget primarily involves domain-specific applications and/or ad hoc architectures, making it hard to disentangle modeling choices from querying strategies \citep{trittenbach2021overview}. 
In contrast, this paper theoretically and empirically studies generalization performance using various labeling budgets, querying strategies, and losses. 

In summary, our main contributions are as follows:
\vspace{-7pt} %
\begin{enumerate}[leftmargin=*,itemsep=-2pt]
\item We prove that the ranking of anomaly scores generalizes from labeled queries to unlabeled data under certain conditions that characterize how well the queries cover the data. Based on this theory, we propose a diverse querying strategy for deep \gls{ad} under labeling budget constraints.

\item We propose \gls{aloe}, a semi-supervised learning framework  compatible with a large number of deep \gls{ad} losses. 
We show how all major hyperparameters can be %
eliminated, making \gls{aloe} easy to use.
To this end, we provide an estimate for the anomaly ratio in the data. 

\item We provide an extensive benchmark for deep \gls{ad} with a limited labeling budget. %
Our experiments on image, tabular, and video data provide evidence that \gls{aloe} outperforms existing methods significantly. Comprehensive ablations disentangle the benefits of each component.


\end{enumerate}

Our paper is structured as follows. \Cref{sec:methods} introduces  the problem setting we address and our main algorithm. \Cref{sec:related} discusses related work in deep \gls{ad}. \Cref{sec:experiments} discusses experimental results on each of image, video, and tabular data. Finally, we conclude this work in Section \ref{sec:discussion}. 



==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/methods.tex <==
\input{figures/toy_example.tex}

\section{Methods}
\label{sec:methods}

\subsection{Notation and Problem Statement}%
\label{sec:prob-setup}
Consider a dataset $\{\vx_i\}_{i=1}^N$ where the datapoints $\vx_i$ are i.i.d. samples from a mixture distribution  $p(\vx)=(1-\alpha)p_0(\vx) + \alpha p_1(\vx)$. The distribution $p_0(\vx)$ corresponds to the normal data, while $p_1(\vx)$ corresponds to anomalous data. We assume that $0 \leq \alpha < 0.5$, i.e., that the anomalous data is non-dominant in the mixture; in practice, $\alpha \ll 0.5$. 

In the \gls{ad} problem, we wish to use the data to train an anomaly detector in the form of a parametric anomaly score function $\s(\vx;\theta)$. Once trained this score function is thresholded to determine whether a datapoint $\vx_i$ is anomalous, as indicated by the binary anomaly label  $y_i := y(\vx_i) \in \{0 := \text{``normal''}, 1:=\text{``abnormal''}\}$.

We focus on the situation where the training data is unlabeled (only $\vx_i$ is known, not $y_i$), but where we have access to an oracle (e.g., a human expert) that is able to provide labels $y_i$ for a budgeted number $K$ of the $N$ training points. 


 

\subsection{Outline of the Technical Approach}

Our work addresses the following questions: How to best select informative data points for labeling -- this is called the {\em querying strategy}, how to best learn an anomaly detector from both the labeled and unlabeled 
data in a semi-supervised fashion, and how to make the approach easy to use by eliminating a crucial hyper-parameter.

\textbf{Querying Strategy.} A successful approach for deep \gls{ad} under labeling budget constraints will require a strategy for selecting the most beneficial set of queries. We choose a theoretically-grounded approach based on generalization performance. For this, we exploit that at test-time an \gls{ad} method will threshold the anomaly scores to distinguish between normal samples and anomalies. This means that the quality of a scoring function is not determined by the absolute anomaly scores but only by their relative ranking. 
In \Cref{sec:active-learning}, we characterize a favorable property of the query set which can guarantee that the ranking of anomaly scores generalizes from the labeled data to unlabeled samples. Since this is desirable, we derive a querying strategy that under a limited labeling budget best fulfills the favorable properties put forth by our analysis. 


\textbf{Semi-supervised Outlier Exposure.} As a second contribution, we propose a semi-supervised learning framework that best exploits both the labeled query set and the unlabeled data. It builds on supervised \gls{ad} and \gls{loe} which we review in \Cref{sec:background}. 
We present \gls{aloe} in \Cref{sec:aloe-loss}. The \gls{aloe} training objective is designed to receive opposing training signals from the normal samples and the anomalies. An EM-style algorithm alternates between estimating the anomaly labels of the unlabaled data and improving the anomaly scoring function using the data samples and their given or estimated labels.

\textbf{Hyperparameter Elimination.} Like related methods discussed in \Cref{sec:related}, \gls{aloe} has an important hyperparameter $\alpha$ which corresponds to the expected fraction of anomalies in the data. While previous work has to assume that $\alpha$ is known \citep{qiu2022latent}, our proposed method presents an opportunity to estimate it. 
The estimate has to account for the fact that the optimal querying strategy derived from our theory in \Cref{sec:active-learning} is not i.i.d.. In \Cref{sec:alpha}, we provide an estimate of $\alpha$ for any stochastic querying strategy.


\subsection{Background: Deep \gls{ad}}
\label{sec:background}
In deep \gls{ad}, 
 auxiliary losses help learn the anomaly scoring function $\s(\vx;\theta)$. Popular losses include autoencoder-based losses \citep{zhou2017anomaly}, the deep SVDD loss \citep{ruff2018deep}, or the neural transformation learning loss \citep{qiu2021neural}. It is assumed that minimizing such a 
 loss $L^\theta_0(\vx)\equiv {\cal L}_0(\s(\vx;\theta))$  over ``normal'' data leads to a desirable scoring function that assigns low scores to normal samples and high scores to anomalies. 

Most deep \gls{ad} methods optimize such an objective over an entire unlabeled data set, even if it contains unknown anomalies. It is assumed that the anomalies are rare enough that they will not dilute the training signal provided by the normal samples ({\em inlier priority}, \citep{wang2019effective}). Building on the ideas of \citet{ruff2019deep} that synthetic anomalies can provide valuable training signal, \citet{qiu2022latent} show how to discover and exploit anomalies by treating the anomaly labels as latent variables in training.

The key idea of \citet{ruff2019deep} is to construct a complementary loss $L^\theta_1(\vx)\equiv {\cal L}_1(\s(\vx;\theta))$ for anomalies that has an opposing effect to the normal loss $L^\theta_0(\vx)$. For example, the deep SVDD loss $L_0^\theta(\vx)=||f_\theta(\vx)-{\bf c}||^2$, with feature extractor $f_\theta$, pulls normal data points towards a fixed center $c$ \citep{ruff2018deep}. The opposing loss for anomalies, defined in \citet{ruff2019deep} as $L_1^\theta(\vx) = 1/L_0^\theta(\vx)$, pushes abnormal data away from the center.

 





\textbf{Supervised \gls{ad}.} Using only the labeled data indexed by $\gQ$ one could train $\s(\vx;\theta)$ using a supervised loss \citep{hendrycks2018deep,gornitz2013toward}
\begin{equation}
\label{eqn:loss}
 {\cal L}_\gQ(\theta) = \frac{1}{|\gQ|}\sum_{j\in \gQ} \big(y_j \La(\vx_j) + (1-y_j) \Ln(\vx_j) \big) .
\end{equation}
\textbf{Latent Outlier Exposure.}
Latent outlier exposure (LOE, \citep{qiu2022latent}) is an unsupervised \gls{ad} framework that uses the same loss as \Cref{eqn:loss} but treats the labels $y$ as latent variables. An EM-style algorithm alternates between optimizing the model w.r.t. $\theta$ and inferring the labels $y$. 


In this work, we propose semi-supervised outlier exposure with a limited labeling budget (SOEL) which builds on these ideas. We next present the querying strategy and \rbt{when the querying strategy leads to correct ranking of anomaly scores (\Cref{sec:active-learning}),} the \gls{aloe} loss (\Cref{sec:aloe-loss}), and how the hyperparameter $\alpha$ can be eliminated (\Cref{sec:alpha})



\subsection{Querying Strategies for \gls{ad}} 
\label{sec:active-learning}

The first ingredient of \gls{aloe} is a querying strategy for selecting informative data points to be labeled,
which we derive from theoretical considerations. %
An important property of the querying strategy is how well it covers unlabeled data. The quality of a querying strategy is determined by the smallest radius $\delta$ such that all unlabeled points are within distance $\delta$ of one queried sample of the same type. In this paper, we prove that if the queries cover both the normal data and the anomalies well (i.e., if $\delta$ is small), a learned anomaly detector that satisfies certain conditions is guaranteed to generalize correctly to the unlabeled data (The exact statement and its conditions will be provided in \Cref{thm:rank}). Based on this insight, we propose to use a querying strategy that is better suited for deep \gls{ad} than previous work.

\input{thms/thm1-ranking}

In \Cref{app:thm1}, we prove \Cref{thm:rank} and discuss the assumptions. An implication of this theorem is that a smaller $\delta$ corresponding to a tighter cover of the data leads to better-generalized ranking performance. As detailed in \Cref{app:thm1}, there is a connection between correct anomaly score ranking and high AUROC performance, a common evaluation metric for \gls{ad}.

Existing methods use querying strategies that do not have good coverage and are therefore not optimal under \Cref{thm:rank}. For a limited querying budget, random querying puts too much weight on high-density areas of the data space, while other strategies only query locally, e.g., close to an estimated decision boundary between normal and abnormal data. 

\textbf{Proposed Querying Strategy.} Based on \Cref{thm:rank}, we propose a querying strategy that encourages tight coverage: diverse querying.
In practice, we use the seeding algorithm of \kmeans which is usually used to initialize diverse clusters.\footnote{This has complexity $O(KN)$ which can be reduced to $O(K\log N)$ using scalable alternatives \citep{bahmani2012scalable}.}  
It iteratively samples another data point to be added to the query set $\gQ$ until the labeling budget is reached. Given the existing queried samples, the probability of drawing another query from the unlabeled set $\gU$ is proportional to its distance to the closest sample already in the query set $\gQ$:
\begin{align}
\label{eq:query-prob}
    p_{\rm query} (\vx_i) = \softmax\big(h(\vx_i)/\tau\big) \quad \forall i \in \gU,
\end{align}
The temperature parameter $\tau$ controls the diversity of the sampling procedure, and  
$h(\vx_i) = \min_{\vx_j \in \mathcal{Q}} d(\vx_i,\vx_j)$ is the distance of a sample $\vx_i$ to the query set $\mathcal{Q}$.
For a meaningful notion of distance, we define $d$ in an embedding space as $d(\vx,\vx') = \|\phi(\vx)-\phi(\vx')\|_2$, where $\phi$ is a neural feature map. We stress that all deep methods considered in this paper have an associated feature map that we can use.
The fact that L2 distance is used in the querying strategy is not an ad-hoc choice but rather aligned with the $\delta$-ball radius definition (\Cref{eq:delta-est} in \Cref{app:thm1}) in \Cref{thm:rank}. 

In \Cref{app:thm1}, we discuss the cover radius and empirically validate that diverse querying leads to smaller $\delta$ than others and is hence advantageous for \gls{ad}.

\subsection{Semi-supervised Outlier Exposure Loss (SOEL)}
\label{sec:aloe-loss}

We next consider how to use both labeled and unlabeled samples in training. We propose \gls{aloe} whose loss combines the unsupervised \gls{ad} loss of LOE~\citep{qiu2022latent} for the unlabeled data with the supervised loss (\Cref{eqn:loss}) for the labeled samples. 
For all queried data (with index set $\gQ$), we assume that ground truth labels $y_i$  are available, while for unqueried data (with index set $\gU$), the labels $\tilde{y}_i$ are unknown. Adding both losses together yields
\begin{align}
\label{eqn:loss-2}
 {\cal L}(\theta, \tilde{\vy}) = \frac{1}{|\gQ|}\sum_{j\in \gQ} \big(y_j \La(\vx_j) + (1-y_j) \Ln(\vx_j) \big) + \nonumber \\ 
 \frac{1}{|\gU|}\sum_{i\in \gU} \big(\tilde{y}_i \La(\vx_i) + (1-\tilde{y}_i) \Ln(\vx_i)\big).
\end{align}
Similar to \citet{qiu2022latent}, optimizing this loss involves a block coordinate ascent scheme that alternates between inferring the unknown labels and taking gradient steps to minimize \Cref{eqn:loss-2} with the inferred labels. In each iteration, the pseudo labels $\tilde{y}_i$ for $i\in \gU$ are obtained by minimizing \Cref{eqn:loss-2} subject to a constraint of $\sum_{i\in\gQ} y_i + \sum_{i\in\gU} \tilde{y}_i = \alpha N$.     
The constraint ensures that the inferred anomaly labels respect a certain contamination ratio $\alpha$. To be specific, let $\tilde\alpha$ denote the fraction of anomalies among the \emph{unqueried} set $\gU$, so that 
$\tilde\alpha |\gU| + \sum_{j\in\gQ}y_j =\alpha N$. 
The constrained optimization problem is then solved by using the current anomaly score function $S$ to rank the unlabeled samples and assign the top $\tilde\alpha$-quantile of the associated labels $\tilde y_i$ to the value $1$, and the remaining to the value $0$. 

We illustrate \gls{aloe}'s effect on a 2D toy data example in \Cref{fig:toy-data}, where \gls{aloe} (\textbf{d}) almost achieves the same performance as the supervised AD (\textbf{c}) with only one queried point.   %


In theory, $\alpha$ could be treated as a hyperparameter, but eliminating hyperparameters is important in \gls{ad}. In many practical applications of \gls{ad}, there is no labeled data that can be used for validation. While \citet{qiu2022latent} have to assume that the contamination ratio is given, \gls{aloe} provides an opportunity to estimate $\alpha$. In \Cref{sec:alpha}, we develop an importance-sampling based approach to estimate $\alpha$ from the labeled data. \rbt{Estimating this ratio can be beneficial for many \gls{ad} algorithms, including OC-SVM~\citep{scholkopf2001estimating}, kNN~\citep{ramaswamy2000efficient}, Robust PCA/Auto-encoder~\citep{zhou2017anomaly}, and Soft-boundary deep SVDD~\citep{ruff2018deep}. When working with contaminated data, these algorithms require a decent estimate of the contamination ratio for good performance.} %


Another noteworthy aspect of the \gls{aloe} loss is that it weighs the \emph{averaged} losses equally to each other. In \Cref{app:ablation_weight}, we empirically show that equal weighting yields the best results among a large range of various weights. This provides more weight to every queried data point than to an unqueried one, because we expect the labeled samples to be more informative. On the other hand, it ensures that neither loss component will dominate the learning task. Our equal weighting scheme is also practical because it avoids a hyperparameter.







\subsection{Contamination Ratio Estimation.}
\label{sec:alpha}
To eliminate a critical hyperparameter in our approach, we estimate the \emph{contamination ratio} $\alpha$, i.e., the fraction of anomalies in the dataset.  Under a few assumptions, we show how to estimate this parameter using mini-batches composed of on non-i.i.d. samples. 

We consider the contamination ratio $\alpha$ as the fraction of anomalies in the data. We draw on the notation from~\Cref{sec:prob-setup} to define $\Ia(\vx)$ as an oracle, outputting $1$ if $\vx$ is an anomaly, and $0$ otherwise (e.g., upon \emph{querying} $\vx$). We can now write $\alpha = \mathbb{E}_{p(\vx)} [\Ia(\vx)]$. 

Estimating $\alpha$ would be trivial given an unlimited querying budget of i.i.d. data samples. The difficulty arises due to the fact that (1) our querying budget is limited, and (2) we query data in a non-i.i.d. fashion so that the sample average is not representative of the anomaly ratio of the full data set. 

Since the queried data points are not independently sampled, we cannot straightforwardly estimate $\alpha$ based on the empirical frequency of anomalies in the query $\gQ$. More precisely, our querying procedure results in a  chain of indices $\gQ = \{i_1, i_2, ..., i_{|\gQ|}\}$, where $i_1 \sim \rm{Unif}(1:N)$, and each conditional distribution $ i_k|i_{<k}$ is defined by \Cref{eq:query-prob}. We will show as follows that this sampling bias can be compensated using importance weights. 
 
As follows, we first propose an importance-weighted estimator of $\alpha$ and then prove the estimator is unbiased under certain idealized conditions specified by two assumptions about our querying strategy. Justifications for the two assumptions will be provided below.

For a random query $\gQ$, its anomaly scores $\{S(\vx_i): i\in\gQ\}$ and anomaly labels $\{\Ia(\vx_i):i\in\gQ\}$ are known. Write $S(\vx_i)$ as $s_i$ and let $p_s(s_i)$ denote the marginal density of population anomaly scores and $q_s(s_i)$ denote the marginal density of the queried samples' anomaly scores. Our importance-weighted estimator of the contamination ratio is
\begin{align}
\label{eq:alpha-is}
    \hat{\alpha} 
    = \frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia(\vx_i). 
\end{align}
As discussed above, $\Ia(\vx_i)$ are the ground truth anomaly labels, obtained from querying $\gQ$. The estimator takes into account that, upon repulsive sampling, we will sample data points in the tail regions of the data distribution more often than we would upon uniform sampling. 

In practice, we learn $p_s$ and $q_s$ using a kernel density estimator in the one-dimensional space of anomaly scores of the training data and the queried data, respectively. We set the bandwidth to the average spacing of scores. With the following two assumptions, \Cref{eq:alpha-is} is unbiased.

\textbf{Assumption 1.} \textsl{The anomaly scores $\{S(\vx_i): i \in \gQ\}$ in a query set $\gQ$ are approximately independently distributed.
}

\textbf{Assumption 2.} \textsl{
Let $\Ia_s(S(\vx))$ denote an oracle that assigns ground truth anomaly labels based on the model's anomaly scores $S(\vx)$.
We assume that such an oracle exists, i.e., the anomaly score $S(\vx)$ is a sufficient statistic of the ground truth anomaly labeling function: $\Ia_s(S(\vx)) = \Ia(\vx)$.}



Assumptions 1 and 2 are only approximations of reality. In our experiment section, we will show that they are good working assumptions to estimate anomaly ratios. Below, we will provide additional strong evidence that assumptions 1 and 2 are well justified. 

The following theorem is a consequence of them:




\input{thms/thm2-alpha}

\rbt{The proof is in \Cref{sec:assum-veri}.} 
\Cref{thm:alpha} allows us to estimate the contamination ratio based on a non-iid query set $\gQ$. 





\textbf{Discussion.} We empirically verified the fact that \Cref{thm:alpha} results in reliable estimates for varying contamination ratios 
in \Cref{app:alpha-est}. Since Assumptions 1 and 2 seem strong, we discuss their justifications and empirical validity next. 

While verifying the independence assumption (Assumption 1) rigorously is difficult, we tested for linear correlations between the scores (\Cref{sec:assum-veri-1}). We found that the absolute off-diagonal coefficient values are significantly smaller than one on CIFAR-10, providing support for Assumption 1. 
A heuristic argument can be provided to support the validity of Assumption 1 based on the following intuition. When data points are sampled diversely in a high-dimensional space, the negative correlations induced by their repulsive nature tend to diminish when the data is projected onto a one-dimensional subspace. This intuition stems from the fact that a high-dimensional ambient space offers ample dimensions for the data points to avoid clustering. To illustrate this, consider the scenario of sampling diverse locations on the Earth's surface, with each location representing a point in the high-dimensional space. By including points from various continents, we ensure diversity in their spatial distribution. However, when focusing solely on the altitude of these locations (such as distinguishing between mountain tops and flat land), it is plausible that the altitude levels are completely uncorrelated. While this heuristic argument provides an intuitive understanding, it is important to note that it does not offer a rigorous mathematical proof.

To test Assumption 2, we tested the degree to which the anomaly score is a sufficient statistic for anomaly scoring on the training set. The assumption would be violated if we could find pairs of training data $\vx_i$ and $\vx_j$, where $\vx_i\neq\vx_j$, with identical anomaly scores $S(\vx_i)=S(\vx_j)$ but different anomaly labels $\Ia_s(s_i)\neq \Ia_s(s_j)$\footnote{The condition $S(\vx_i)\neq S(\vx_j)$ for $\vx_i\neq\vx_j$ hints we can assign a unique label to each data point based on their scores.}. On FMNIST, we found 38 data pairs with matching scores, and none of them had opposite anomaly labels. For CIFAR-10, the numbers were 21 and 3, respectively. See \Cref{sec:assum-veri-3} for details. 







==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/sections/related-work.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Deep Anomaly Detection.}
Many recent advances in anomaly detection are in the area of deep learning \citep{ruff2021unifying}. One early strategy was to use autoencoder- \citep{principi2017acoustic,zhou2017anomaly} or density-based models \citep{schlegl2017unsupervised, deecke2018image}. Another pioneering stream of research combines one-class classification \citep{scholkopf2001estimating} with deep learning for unsupervised \citep{ruff2018deep,ijcai2022p305} and semi-supervised \citep{ruff2019deep} anomaly detection. Many other approaches to deep anomaly detection are self-supervised. %
They employ a self-supervised loss function to train the detector and score anomalies \citep{golan2018deep,hendrycks2019using,bergman2020classification,qiu2021neural,shenkar2022anomaly,schneider2022detecting}. Our work resides in the self-supervised anomaly detection category and can be extended to other data modalities if an appropriate loss is provided.%

While all these methods assume that the training data consists of only normal samples, in many practical applications, the training pool may be contaminated with unidentified anomalies \citep{vilhjalmsson2013nature,poisoning1}.
This can be problematic because the detection accuracy typically deteriorates when the contamination ratio increases \citep{wang2019effective}. Addressing this, refinement \citep{zhou2017anomaly,yoon2021self} attempts to cleanse the training pool by removing anomalies therein, although they may provide valuable training signals. As a remedy, \citet{qiu2022latent} propose to jointly infer binary labels to each datum (normal vs. anomalous) while updating the model parameters based on outlier exposure. Our work also makes the contaminated data assumption and employs the training signal of abnormal data.

\textbf{Querying Strategies for Anomaly Detection.} Querying strategies play an important role in batch active learning \citep{sener2018active, ash2020deep, citovsky2021batch, pinsler2019bayesian, hoi2006large} but are less studied for anomaly detection.
The human-in-the-loop setup for anomaly detection has been pioneered by \citet{pelleg2004active}. %
Query samples are typically chosen locally, e.g., close to the decision boundary of a one-class SVM \citep{gornitz2013toward,yin2018active} or sampled according to a density model \citep{ghasemi2011active}. \citet{siddiqui2018feedback,das2016incorporating} propose to query the most anomalous instance, while \citet{das2019active} employ a tree-based ensemble to query both anomalous and diverse samples. A recent survey compares various aforementioned query strategies with one-class classifiers \citep{trittenbach2021overview}.

\citet{pimentel2020deep} query samples with the top anomaly scores for autoencoder-based methods, while \citet{ning2022deep} improve the querying by considering the diversity. \citet{tang2020deep} use an ensemble of deep anomaly detectors and query the most likely anomalies for each detector separately. \citet{russo2020active} query samples where the model is uncertain about the predictions. \citet{pang2021toward} and \citet{zha2020meta} propose querying strategies based on reinforcement learning, which requires labeled datasets. 

All these querying strategies do not optimize coverage as defined in \Cref{thm:rank}, and as a result, their generalization guarantees are less favorable than our method.   
Most querying strategies from the papers discussed above are fairly general and can be applied in combination with various backbone models. 
Since more powerful backbone models have been released since these earlier publications, we ensure a fair comparison by studying all querying strategies in combination with the same backbone models as \gls{aloe}.







==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/ablation-backbone.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{$|\gQ|=20$. AUC ($\%$) with standard deviation for anomaly detection on CIFAR-10 and F-MNIST. For all experiments, we set the contamination ratio as $10\%$. \gls{aloe} mitigates the performance drop when \gls{ntl} and \gls{mhrot} trained on the contaminated datasets. Results of the unsupervised method LOE are borrowed from \citet{qiu2022latent}.}
	\label{tab:ablation-backbone}
	\small
	\centering
	\vspace{1pt}
	
	\begin{tabular}{l@{\hskip 0.3in}cccc@{\hskip 0.3in}ccc}
        \toprule
        & \multicolumn{3}{c}{NTL} & & 
        \multicolumn{3}{c}{MHRot} \\
        \cmidrule(r){2-4} \cmidrule(r){6-8}
        & LOE & \kmeans & \gls{aloe} & & LOE & \kmeans & \gls{aloe} \\
		\cmidrule(r){2-4} \cmidrule(r){6-8}
		CIFAR-10 & 94.9$\pm$0.1 &95.6$\pm$0.3 &\textbf{96.3$\pm$0.3}& &86.3$\pm$0.2 &64.0$\pm$0.2 &\textbf{86.9$\pm$0.7}  \\ 
		F-MNIST &92.5$\pm$0.1 &94.3$\pm$0.2 &\textbf{94.8$\pm$0.4}& &91.2$\pm$0.4 &91.5$\pm$0.1 &\textbf{92.6$\pm$0.1} \\
        \bottomrule
	\end{tabular}
	
\end{table}




==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/ablation-pseudo-y.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{Performance of ablation study on $\tilde y$. AUROC (\%) on CIFAR-10 and F-MNIST when $|\gQ|=20$, the ground-truth contamination ratio is 0.1, and the backbone model is NTL. } %
	\label{tab:ablation-pseudo-y}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lcccccc}
        \toprule
		$\tilde y$ & 1.0 &0.875  &0.75 &0.625 &0.5 &0.25   \\
		\midrule
		CIFAR-10 &95.3 $\pm$ 0.6  &95.7 $\pm$ 0.4  &95.8 $\pm$ 0.4 &96.0 $\pm$ 0.5 &96.3 $\pm$ 0.3 &94.5 $\pm$ 0.3  \\
		F-MNIST & 94.5  $\pm$ 0.5  &94.5 $\pm$ 0.4  &94.6 $\pm$ 0.4 &94.6 $\pm$ 0.3 &94.8 $\pm$ 0.6 &94.0 $\pm$ 0.4\\
        \bottomrule
	\end{tabular}
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/ablation-tau.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{Performance of ablation study on $\tau$. AUROCs (\%) on CIFAR-10 and F-MNIST when $|\gQ|=20$, the ground-truth contamination ratio is 0.1, and the backbone model is NTL. } %
	\label{tab:ablation-tau}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lcccc}
        \toprule
		   $\tau$  & 1 & 0.1 & 0.01 & 0.001  \\
		\midrule
		CIFAR-10 &$93.2 \pm 1.7$  & $94.5 \pm 0.8$  & $96.3 \pm 0.3$ & $95.9 \pm 0.4$  \\
		F-MNIST & $91.8 \pm 1.4$ & $92.7 \pm 1.1$ & $94.8 \pm 0.6$ & $94.9 \pm 0.2$ \\
        \bottomrule
	\end{tabular}
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/contamination-ratio.tex <==



\begin{table}[ht]
\vspace{-5pt}
	\caption{Estimated contamination ratios on CIFAR-10 and F-MNIST when $|\gQ|=40$ and the backbone model is NTL. The first row shows the true contamination ratio ranging from $1\%$ to $45\%$. The estimations are repeated 50 times.} %
	\label{tab:alpha-estimate}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lccccc}
        \toprule
		     & 1\% & 5\% & 10\% & 15\% &20\% \\
		\midrule
		CIFAR-10 &$0.5\% \pm 1.2\%$ & $6.0\% \pm 3.3\%$ & $12.0\% \pm 4.4\%$ & $15.3\% \pm 4.5\%$ 
        & 18.9\% $\pm$ 5.4\%\\
		F-MNIST &$1.0\% \pm 1.5\%$ & $3.8\% \pm 2.3\%$ &  $8.7\% \pm 4.1\%$ & $12.8\% \pm 5.3\%$ 
        & 19.3\% $\pm$ 5.1\%\\
        \bottomrule
	\end{tabular}

        \begin{tabular}{lccccc}
        \toprule
		     &25\% &30\% &35\% &40\% &45\% \\
		\midrule
		CIFAR-10 &26.2\% $\pm$ 6.0\%   & 30.6\% $\pm$ 5.5\% &35.8\% $\pm$ 6.9\%  &42.0\% $\pm$ 7.7\%  &47.2\% $\pm$ 6.7\%\\
		F-MNIST &27.9\% $\pm$ 6.4\%  &31.8\% $\pm$ 6.1\% &38.3\% $\pm$ 6.5\% &43.1\% $\pm$ 5.7\% &48.9\% $\pm$ 5.6\% \\
        \bottomrule
	\end{tabular}
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/dsvdd-mhrot-image.tex <==
\begin{table}[ht]
	\caption{$|\gQ|=20$. AUC ($\%$) with standard deviation for anomaly detection on six datasets (CIFAR-10, F-MNIST, Blood, OrganA, OrganC, OrganS). The backbone models are \gls{mhrot}~\citep{hendrycks2019using} and Deep SVDD~\citep{ruff2018deep}. For all experiments, we set the contamination ratio as $10\%$. \gls{aloe} consistently outperforms two best-performing baselines on all six datasets.}
	\label{tab:backbone-dsvdd-mhrot}
	\small
	\centering
	\vspace{1pt}
	
	\begin{tabular}{l@{\hskip 0.3in}cccc@{\hskip 0.3in}ccc}
        \toprule
        & \multicolumn{3}{c}{MHRot} & & 
        \multicolumn{3}{c}{Deep SVDD} \\
        \cmidrule(r){2-4} \cmidrule(r){6-8}
        & \gls{aloe} & \HybridA & \HybridB & & \gls{aloe} & \HybridA & \HybridB \\
		\cmidrule(r){2-4} \cmidrule(r){6-8}
		CIFAR-10 & \textbf{86.9$\pm$0.7} & 83.9$\pm$0.1 & 49.1$\pm$2.0 && \bf93.1$\pm$0.2 & 89.0$\pm$0.6 & 91.3$\pm$1.0 \\ 
		F-MNIST &\textbf{92.6$\pm$0.1} & 87.1$\pm$0.2 & 58.9$\pm$5.7 && \bf91.4$\pm$0.5 & 90.9$\pm$0.4 & 82.5$\pm$2.9\\
        Blood &\textbf{83.3$\pm$0.2} & 81.1$\pm$2.5 & 61.8$\pm$2.1 && \bf80.2$\pm$1.1 & 79.7$\pm$1.2 & 77.2$\pm$3.0\\
        OrganA & \textbf{96.5$\pm$0.3} & 94.1$\pm$0.3 & 61.1$\pm$4.8 && \bf89.5$\pm$0.3 & 87.1$\pm$0.7 & 71.3$\pm$3.8\\
        OrganC & \textbf{92.1$\pm$0.2} & 91.6$\pm$0.1 & 70.9$\pm$0.8  && \bf87.5$\pm$0.7 & 85.3$\pm$0.8 & 84.2$\pm$0.9\\
        OrganS & \textbf{89.3$\pm$0.2} & 88.3$\pm$0.3 & 68.2$\pm$0.1  && \bf85.5$\pm$0.7 & 83.4$\pm$0.3 & 81.2$\pm$1.3\\
        \bottomrule
	\end{tabular}
	
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/hyperparameters.tex <==
\begin{table}[ht]
    \centering
    \small
    \begin{tabular}{ll|cccc}
    \toprule
    Model & Dataset &  Learning Rate & Epoch & Minibatch Size & $\tau$\\
    \midrule
    \multirow{5}{*}{NTL} & CIFAR-10 &  1e-4 & 30 & 512 & 1e-2 \\
        & F-MNIST &  1e-4 & 30 & 512 & 1e-2 \\
        & MedMNIST & 1e-4 & 30 & 512 & 1e-2 \\
        & ODDS & 1e-3 & 100 & $\lceil N/5 \rceil$ & 1e-2 \\
        & UCSD Peds1 & 1e-4 & 3$^*$ & 192 & 1e-2 \\
    \midrule
    \multirow{3}{*}{MHRot} & CIFAR-10 &  1e-3 & 15 & 10 & N/A \\
        & F-MNIST &  1e-4 & 15$^{**}$ & 10 & N/A \\
        & MedMNIST &  1e-4 & 15 & 10 & N/A \\
    \midrule
    \multirow{3}{*}{Deep SVDD} & CIFAR-10 & 1e-4 & 30 & 512 & 1e-2  \\
        & F-MNIST  & 1e-4 & 30 & 512 & 1e-2\\
        & MedMNIST & 1e-4 & 30 & 512 & 1e-2 \\
    \bottomrule
    \multicolumn{5}{l}{{\small $^*$\HybridB, \HybridC, \PositiveB, and \PositiveA~train 30 epochs. All other methods train 3 epochs.}}\\
    \multicolumn{5}{l}{{\small $^{**}$\gls{aloe} train 3 epochs. }}
    \end{tabular}
    \caption{A summary of optimization parameters for all methods.}
    \label{tab:opt-param}
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/knn-comparison.tex <==
\begin{table}[ht]
\vspace{-5pt}
    \caption{Comparisons with kNN method. We reported the F1-score ($\%$) with standard error for anomaly detection on tabular datasets when the query budget $K=10$. \gls{aloe} outperforms the kNN baseline. }
\label{tab:tab_knn}
    \centering
    \small
  \begin{tabular}{l|cc}
  \toprule
     & \bfseries $k^{\text{th}}$NN & \bfseries ALOE \\ 
  \midrule
\bfseries  BreastW  & 92.5$\pm$2.1	& \textbf{93.9$\pm$0.5}	\\ 
\bfseries Ionosphere & 88.1$\pm$1.3	& \textbf{91.8$\pm$1.1}	\\ 
 \bfseries Pima & 40.5$\pm$4.7	& \textbf{55.5$\pm$1.2}	\\ 
 \bfseries Satellite & 61.1$\pm$2.2	& \textbf{71.1$\pm$1.7}	\\ 
\midrule
\bfseries Average & 70.6 & \textbf{78.1} \\
  \bottomrule 
  \end{tabular}
 \vspace{-5pt}
\end{table}


==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/methods.tex <==

\begin{table*}[t!]
\vspace{-5pt}
	\caption{A summary of all compared experimental methods' query strategy and training strategy irrespective of their backbone models.}
	\label{tab:baselines}
 	\footnotesize
	\centering
	\begin{tabular}{lll@{\hskip 0.2in}cc}
        \toprule
		Name & Reference & Querying Strategy & Loss (labeled) & Loss (unlabeled)  \\
		\midrule
		\Margin & \citet{gornitz2013toward}  &margin query %
		& superv. (\Cref{eqn:loss}) & one class \\
        \HybridA & \citet{gornitz2013toward} & margin diverse query %
        & \ditto & one class  \\
        \PositiveB & \citet{pimentel2020deep} & most positive query & \ditto & none \\
        \PositiveA & \citet{barnabe2015active} & most positive query & \ditto & one class \\
        
        \RandomA & \citet{ruff2019deep} & random query & \ditto & one class  \\
        \RandomB & \citet{trittenbach2021overview} & positive random query & \ditto & one class    \\
        \HybridB &\citet{das2019active} &positive diverse query & \ditto & none \\
        \HybridC & \citet{ning2022deep} &positive diverse query & refinement & weighted one class \\
        \midrule
        SOEL& [ours] & diverse (\Cref{eq:query-prob}) & \multicolumn{2}{c}{ semi-supervised outlier exposure loss (\Cref{eqn:loss-2})} \\
        \bottomrule
	\end{tabular}
 	\vspace{-5pt}
\end{table*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/results.tex <==





\begin{table*}[t!]
\vspace{-5pt}
    \caption{AUC ($\%$) with standard deviation for anomaly detection on 11 image datasets when the query budget $|\gQ|=20$. \gls{aloe} outperforms all baselines by a large margin by querying diverse and informative samples.}%
\label{tab:img_results}
    \footnotesize
    \centering
  \begin{tabular}{l|ccccccccc}
  \toprule
     & \bfseries\Margin & \bfseries\HybridA & \bfseries\PositiveB & \bfseries\PositiveA & \bfseries\RandomA & \bfseries\RandomB & \bfseries\HybridB & \bfseries\HybridC & \bfseries SOEL \\ 
  \midrule
    \bfseries CIFAR10                  & 92.4$\pm$0.7                                    & 92.0$\pm$0.7                                     & 93.4$\pm$0.5                                       & 92.1$\pm$0.7                                       & 89.2$\pm$3.2                                     & 91.4$\pm$1.0                                     & 85.1$\pm$2.2                                     & 71.8$\pm$7.4                                     & \textbf{96.3$\pm$0.3}                  \\ 
\bfseries FMNIST                   & 93.1$\pm$0.4                                    & 92.6$\pm$0.4                                     & 92.2$\pm$0.6                                       & 89.3$\pm$1.0                                       & 84.0$\pm$3.8                                     & 90.6$\pm$1.1                                     & 88.7$\pm$1.4                                     & 82.6$\pm$4.3                                     & \textbf{94.8$\pm$0.6}                  \\ 
\bfseries Blood                    & 68.6$\pm$1.8                                    & 69.1$\pm$1.3                                     & 69.6$\pm$1.8                                       & 72.2$\pm$4.9                                       & 70.6$\pm$1.6                                     & 69.2$\pm$1.7                                     & 72.2$\pm$2.7                                     & 58.3$\pm$5.2                                     & \textbf{80.5$\pm$0.5}                  \\ 
\bfseries OrganA                   & 86.4$\pm$1.3                                    & 87.4$\pm$0.7                                     & 81.7$\pm$2.9                                       & 81.8$\pm$2.1                                       & 82.9$\pm$0.6                                     & 86.5$\pm$0.7                                     & 88.6$\pm$1.5                                     & 68.8$\pm$3.1                                     & \textbf{90.7$\pm$0.7}                  \\ 
\bfseries OrganC                   & 86.5$\pm$0.9                                    & 87.0$\pm$0.7                                     & 84.6$\pm$1.9                                       & 79.6$\pm$2.0                                       & 85.5$\pm$0.9                                     & 86.4$\pm$0.8                                     & 84.8$\pm$1.2                                     & 68.9$\pm$3.0                                     & \textbf{89.7$\pm$0.7}                  \\ 
\bfseries OrganS                   & 83.5$\pm$1.1                                    & 84.1$\pm$0.4                                     & 83.2$\pm$1.3                                       & 78.6$\pm$1.0                                       & 82.2$\pm$1.4                                     & 83.8$\pm$0.4                                     & 82.3$\pm$0.7                                     & 66.9$\pm$4.3                                     & \textbf{87.4$\pm$0.8}                  \\ 
\bfseries OCT                      & 64.4$\pm$3.7                                    & 63.3$\pm$1.8                                     & 63.8$\pm$4.4                                       & 63.0$\pm$4.0                                       & 59.7$\pm$1.9                                     & 62.1$\pm$4.3                                     & 63.0$\pm$7.6                                     & 56.2$\pm$4.5                                     & \textbf{68.5$\pm$3.4}                  \\ 
\bfseries Path                     & 82.7$\pm$2.4                                    & 86.0$\pm$1.1                                     & 77.5$\pm$2.0                                       & 80.2$\pm$3.5                                       & 83.2$\pm$1.6                                     & 83.9$\pm$2.9                                     & 86.1$\pm$2.0                                     & 75.1$\pm$4.2                                     & \textbf{88.1$\pm$1.1}                  \\ 
\bfseries Pneumonia                & 72.1$\pm$7.0                                    & 75.1$\pm$5.3                                     & 75.5$\pm$8.8                                       & 83.6$\pm$6.1                                       & 68.1$\pm$5.9                                     & 76.0$\pm$8.0                                     & 88.4$\pm$3.3                                     & 63.4$\pm$17.7                                    & \textbf{91.2$\pm$1.4}                  \\ 
\bfseries Tissue                   & 60.2$\pm$1.5                                    & 61.3$\pm$1.7                                     & 65.8$\pm$1.7                                       & 63.5$\pm$2.0                                       & 59.9$\pm$1.7                                     & 59.5$\pm$1.3                                     & 62.1$\pm$1.7                                     & 50.8$\pm$1.6                                     & \textbf{66.4$\pm$1.4}                  \\ 
\bfseries Derma                    & 62.6$\pm$3.8                                    & 63.1$\pm$4.7                                     & 66.6$\pm$2.3                                       & 66.4$\pm$4.3                                       & 64.5$\pm$4.8                                     & 68.3$\pm$2.1                                     & 57.2$\pm$13.3                                    & 48.0$\pm$13.6                                    & \textbf{73.5$\pm$2.5}                  \\ 
\midrule
\bfseries Average & 77.5 & 78.3 &  77.3  & 77.6 &75.4 &78.0 &78.0 &64.6 &\textbf{84.3} \\
  \bottomrule 
  \end{tabular}
 
\vspace{-5pt}
\end{table*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/tabular.tex <==






\begin{table*}[t!]
\vspace{-5pt}
    \caption{F1-score ($\%$) with standard deviation for anomaly detection on tabular data when the query budget $|\gQ|=10$. \gls{aloe} performs the best on 3 of 4 datasets and outperforms all baselines by 3.2 percentage points on average.}%
\label{tab:tab_results}
    \footnotesize
    \centering
  \begin{tabular}{l|ccccccccc}
  \toprule
     & \bfseries\Margin & \bfseries\HybridA & \bfseries\PositiveB & \bfseries\PositiveA & \bfseries\RandomA & \bfseries\RandomB & \bfseries\HybridB & \bfseries\HybridC & \bfseries \gls{aloe} \\ 
  \midrule
\bfseries  BreastW  & 81.6$\pm$0.7	& 83.3$\pm$2.0	& 58.6$\pm$7.7	& 81.3$\pm$0.8	& 87.1$\pm$1.0	& 82.9$\pm$1.1	& 55.0$\pm$6.0	& 79.6$\pm$4.9	& \textbf{93.9$\pm$0.5}	\\ 
\bfseries Ionosphere & 91.9$\pm$0.3	& \textbf{92.3$\pm$0.5}	& 56.1$\pm$6.2	& 91.1$\pm$0.8	& 91.1$\pm$0.3	& 91.9$\pm$0.6	& 64.0$\pm$4.6	& 88.2$\pm$0.9	& 91.8$\pm$1.1	\\ 
 \bfseries Pima & 50.1$\pm$1.3	& 49.2$\pm$1.9	& 48.5$\pm$0.4	& 52.4$\pm$0.8	& 53.6$\pm$1.1	& 51.9$\pm$2.0	& 53.8$\pm$4.0	& 48.4$\pm$0.7	& \textbf{55.5$\pm$1.2}	\\ 
 \bfseries Satellite & 64.2$\pm$1.2	& 66.2$\pm$1.7	& 57.0$\pm$3.0	& 56.7$\pm$3.2	& 67.7$\pm$1.2	& 66.6$\pm$0.8	& 48.6$\pm$6.9	& 56.9$\pm$7.0	& \textbf{71.1$\pm$1.7}	\\ 
\midrule
\bfseries Average & 72.0 & 72.8 & 55.1 & 70.4 & 74.9 & 73.3 & 55.4 &  68.3 & \textbf{78.1} \\
  \bottomrule 
  \end{tabular}
 \vspace{-10pt}
\end{table*}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/tables/tabular_benchmark.tex <==
\begin{table}[ht]
    \caption{F1-scores (in $\%$) and their standard deviations of 13 anomaly detection methods on tabular data. Results are taken from \citet{alvarez2022revealing}. The results indicate that NTL is the state-of-the-art for tabular anomaly detection.}
\label{tab:tab_benchmark}
 	\small
    \centering
  \begin{tabular}{l|ccccc|c}
  \toprule
     & KDDCUP10 & NSL-KDD & IDS2018& Arrhythmia & Thyroid & Avg.\\ 
  \midrule
ALAD & 95.9$\pm$0.7 & 92.1$\pm$1.5 & 59.0$\pm$0.0 & 57.4$\pm$0.4& 68.6$\pm$0.5 & 74.6  \\         
DAE & 93.2$\pm$2.0 &\bf96.1$\pm$0.1 &\bf71.5$\pm$0.5 & 61.5$\pm$2.5 & 59.0$\pm$1.5 & 76.3 \\
DAGMM & 95.9$\pm$1.4 &85.3$\pm$7.4 &55.8$\pm$5.3 & 50.6$\pm$4.7 & 48.6$\pm$8.0 & 67.2 \\
DeepSVDD &89.1$\pm$2.0 &89.3$\pm$2.0 &20.8$\pm$11 & 55.5$\pm$3.0&  13.1$\pm$13 & 53.6 \\
DROCC & 91.1$\pm$0.0 &90.4$\pm$0.0 &45.6$\pm$0.0 & 35.8$\pm$2.6 & 62.1$\pm$10 & 65.0 \\
DSEBM-e & 96.6$\pm$0.1 &94.6$\pm$0.1 &43.9$\pm$0.8 & 59.9$\pm$1.0 & 23.8$\pm$0.7 & 63.8 \\
DSEBM-r & \bf98.0$\pm$0.1 &95.5$\pm$0.1 &40.7$\pm$0.1 & 60.1$\pm$1.0 & 23.6$\pm$0.4 & 63.6 \\
DUAD & 96.5$\pm$1.0 &94.5$\pm$0.2 &\bf71.8$\pm$2.7 & 60.8$\pm$0.4 & 14.9$\pm$5.5 & 67.7 \\
MemAE &95.0$\pm$1.7 &95.6$\pm$0.0 &59.9$\pm$0.1 & 62.6$\pm$1.6& 56.1$\pm$0.9 & 73.8 \\
SOM-DAGMM &97.7$\pm$0.3 &95.6$\pm$0.3 &44.1$\pm$1.1 & 51.9$\pm$5.9 & 52.7$\pm$12 & 68.4 \\
LOF &95.1$\pm$0.0 &91.1$\pm$0.0 &63.8$\pm$0.0 & 61.5$\pm$0.0 & 68.6$\pm$0.0 & 76.0 \\
OC-SVM &96.7$\pm$0.0 &93.0$\pm$0.0 &45.4$\pm$0.0 & \bf63.5$\pm$0.0 & 68.1$\pm$0.0 &  73.3 \\
NTL &96.4$\pm$0.2 &\bf96.0$\pm$0.1 &59.5$\pm$8.9 & 60.7$\pm$3.7 & \bf73.4$\pm$0.6 & \bf77.2 \\
  \bottomrule 
  \end{tabular}
\end{table}

==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/thms/proof-thm2.tex <==
\begin{proof}
\vspace{-0.5em}
Let A1 and A2 denote Assumption 1 and 2, respectively. Furthermore, 
let $q(\vx_1, ..., \vx_{|\gQ|})$ and $q_s(s_1, ..., s_{|\gQ|})$ denote the query distribution in the data and anomaly score spaces, respectively. A2 assumes $\Ia_s(s):=\Ia_s(S(\vx))=\Ia(\vx)$ for all $\vx$. So the expectation of \Cref{eq:alpha-is} is 
\begin{align*}
&\E[\hat \alpha] = \E_{q(\vx_1, ..., \vx_{|Q|})}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(S(\vx_i))}{q_s(S(\vx_i))}\Ia(\vx)\right]  
\stackrel{A2}{=} \E_{q_s(s_1, ..., s_{|Q|})}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right] \\ 
& \stackrel{A1}{=} \E_{\prod_{i=1}^{|Q|}q_s(s_i)}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right] 
= \frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|} \E_{q_s(s_i)}\left[\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right]
= \E_{p_s(s)}[\Ia_s(s)] \\
&= \E_{p(\vx)}[\Ia_s(S(\vx))]
\stackrel{A2}{=}\E_{p(\vx)}[\Ia(\vx)]=\alpha
\end{align*}
where the change of variables makes necessary assumptions, including the existence of density functions. \qedhere 


\vspace{-0.5em}
\end{proof}

















==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/thms/thm1-ranking.tex <==

\begin{theorem}
\label{thm:rank}
Let $\gQ_0$ be the index set of datapoints labeled normal and $\gQ_1$ the index set of datapoints labeled abnormal. 
Let $\delta \in \mathbb{R}^+$ be the smallest radius, such that for each unlabeled anomaly $\vu_a$ and each unlabeled normal datum $\vu_n$ there exist labeled data points $\vx_a, a\in\gQ_1$ and $\vx_n, n\in\gQ_0$, such that $\vu_a$ is within the $\delta$-ball of $\vx_a$ and $\vu_n$ is within the $\delta$-ball around  $\vx_n$. If a $\lambda_s$-Lipschitz continuous function $\s$ ranks the labeled data correctly, with a large enough margin, i.e. $\s(\vx_a)-\s(\vx_n) \geq 2\delta\lambda_s$,
then $\s$ ranks the unlabeled points correctly, too, and $\s(\vu_a)%
\geq\s(\vu_n)$.
\end{theorem}


==> Deep_Active_Anomaly_Detection_--_ICML_2023_arXiv/thms/thm2-alpha.tex <==
\begin{theorem}
\label{thm:alpha}
Assume that Assumptions 1 and 2 hold. Then, \Cref{eq:alpha-is} is an unbiased estimator of the contamination ratio $\alpha$, i.e., $\E[\hat\alpha]=\alpha$.



\end{theorem}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/ablation-weight.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/cifar_query_weight.pdf}
    \includegraphics[width=0.45\linewidth]{images/fmnist_query_weight.pdf}
    \caption{Ablation study on the weighting scheme in \Cref{eqn:loss-2}. With different query budgets $|\gQ|$, the performance on image datasets degrades both upon down-weighting (0.01, 0.1) or up-weighting (10.0) the queried samples. In contrast, equal weighting yields optimal results. } 
    \label{fig:ablation-weight}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/ablation_query.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=1\linewidth]{images/query_comp_new_legend.pdf}
    \caption{Ablation study on the query strategy. K-Means++ significantly outperforms other strategies for active anomaly detection on most of the datasets.} 
    \label{fig:ablation-query}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/ablation_true_est_ratio.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{images/true_est_ratio_comp_new_legend.pdf}
    \vspace{-10pt}
    \caption{Model using the estimated ratio is indistinguishable from the one using the true ratio.} 
    \label{fig:ablation-true-est-ratio}
\end{figure}



==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/corr_mat.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\linewidth]{images/corr_mat_cifar10_0.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_cifar10_1.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_fmnist_0.pdf}
    \includegraphics[width=0.4\linewidth]{images/corr_mat_fmnist_1.pdf}
    \caption{Anomaly score correlation matrix $\langle S(\vx_i),S(\vx_j)\rangle$, where $\vx_i$ and $\vx_j$ are jointly sampled in the same query set. The result indicates that anomaly scores can be considered as approximately independent random variables.
    } 
    \label{fig:corr-mat}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/grad-diverse-comparison.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/grad_diverse_compare_cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/grad_diverse_compare_fmnist.pdf}
    \caption{Comparison with gradient diversity querying strategy (BADGE)~\citep{ash2020deep}. The gradients wrt. the penultimate layer representation don't provide as informative queries as the representation itself, thus outperformed by our querying strategy \gls{aloe}. The true contamination ratio is 10\%.} 
    \label{fig:grad-div-comparison}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/image_benchmark.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.85\linewidth]{images/error_years.png}
  \caption{Error (in $\%$ of 1-AUCROC) of ten methods on CIFAR10: two shallow methods (SVDD \citep{TaxD04} and IF \citep{liu2008isolation}) and eight deep methods (VAE \citep{kingma2014vae}, DCAE \citep{makhzani2015winner}, ADGAN \citep{deecke2018image}, DSVDD \citep{ruff2018deep}, GT \citep{golan2018deep}, MHRot \citep{hendrycks2019using}, Contrastive \citep{sohn2020learning}, and NTL \citep{qiu2022latent}). \gls{ntl} achieves the best anomaly detection performance on CIFAR10.
    \label{fig:image_benchmark}}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/image_data.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/img_res_font+_new_legend.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs the best among the compared methods on all query budgets.}
    \label{fig:img_data}
\vspace{-10pt}
\end{figure*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/image_data_batch_seq.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.7\linewidth]{images/img_res_seq.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs better than a sequential version.}
    \label{fig:img-data-seq}
\vspace{-10pt}
\end{figure*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/image_data_comparison_bce.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{images/img_res_bce.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets. Models are evaluated at $20, 40, 80, 160$ queries. Deep \gls{ad} model (\gls{ntl}) performs significantly better than a binary classifier.}
    \label{fig:img-data-bce}
\vspace{-10pt}
\end{figure*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/robust-ratio.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.01.pdf}
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.05.pdf}
    \includegraphics[width=0.5\linewidth]{images/img_res_ratio0.2.pdf}
    \vspace{-10pt}
    \caption{Running AUCs (\%) with different query budgets and data contamination ratios (1\%-top row, 5\%-middle row, 20\%-bottom row). Models are evaluated at $20, 40, 80, 160$ queries. \gls{aloe} performs the best on all three contamination ratio setups.}
    \label{fig:robust-ratio}
\vspace{-10pt}
\end{figure*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/semisuper-comparison.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/semisuper_compare_cifar10_new_legend.pdf}
    \includegraphics[width=0.45\linewidth]{images/semisuper_compare_fmnist_new_legend.pdf}
    \caption{Comparison with semi-supervised learning fraemworks, FixMatch \citep{sohn2020fixmatch}, $k$-nearest neighbors \citep{iscen2019label}, and Gaussian process \citep{li2018pseudo}. On F-MNIST, \gls{aloe} outperforms all baselines, while on CIFAR-10, \gls{aloe} has a comparable performance with FixMatch with \kmeans querying.} 
    \label{fig:semisuper-comparison}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/thm1-delta.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/thm1_check_delta_cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/thm1_check_delta_fmnist.pdf}
    \caption{Cover radius $\delta$ (\Cref{eq:delta-est}) resulted from different querying strategies on the first class of CIFAR-10 and F-MNIST. Diverse queries systematically have smaller cover radius than other querying strategies.} 
    \label{fig:thm1-delta}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/thm1-ranking.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\linewidth]{images/rank-unlabeled-cifar10.pdf}
    \includegraphics[width=0.45\linewidth]{images/rank-unlabeled-fmnist.pdf}
    \caption{Ranking performance of unlabeled data. AUC of unqueried data is evaluated using the fitted anomaly detector on the queried data. Our proposed diverse querying (\kmeans) provides better ranking of the unlabeled data.} 
    \label{fig:ranking-unquery}
\end{figure}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/toy_example.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/toy_example_fewer_query_new_order_v2.pdf}
    \vspace{-10pt}
    \caption{Anomaly score contour plots on 2D toy data demonstrate that \gls{aloe} [ours, (\textbf{d})] with only one labeled sample can achieve detection accuracy that is competitive with a fully supervised approach (\textbf{a}). Binary classification (\textbf{b}) is problematic for \gls{ad} since it cannot detect new anomalies, e.g. in the upper right corner of the plot. Subplot (\textbf{c}) demonstrates that unsupervised \gls{ad} is challenging with contaminated data. Even a single labeled query, in combination with our approach, can significantly improve \gls{ad}.}
    
    \label{fig:toy-data}
\vspace{-10pt}
\end{figure*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/figures/video_data.tex <==
\begin{figure}[ht]
\vspace{-10pt}
    \centering
    \includegraphics[width=0.85\linewidth]{images/video_res_c3e-1_font+_new_legend_wide.pdf}
\vspace{-10pt}
    \caption{Results on the video dataset UCSD Peds1 with different query budgets. \gls{aloe} achieves the leading performance.
    } 
    \label{fig:video_data}
 \vspace{-10pt}
\end{figure}



==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/header.tex <==
\PassOptionsToPackage{numbers, sort&compress}{natbib}

\usepackage[accepted]{icml2023}



\usepackage[utf8]{inputenc} %
\usepackage[T1]{fontenc}    %
\usepackage[hidelinks]{hyperref}  
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{xcolor}         %
\usepackage{multirow}
\usepackage[pdftex]{graphicx}
\usepackage{dsfont}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{float}
\bibliographystyle{unsrtnat}


\usepackage{xr-hyper}
\newcommand{\theHalgorithm}{\arabic{algorithm}}

\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}


\usepackage{glossaries-extra}
\setabbreviationstyle[acronym]{long-short}
\glssetcategoryattribute{acronym}{nohyperfirst}{true}
\renewcommand*{\glsdonohyperlink}[2]{%
 {\glsxtrprotectlinks \glsdohypertarget{#1}{#2}}}
\usepackage{xfrac}
\input{math-commands}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\def\Ln{L_0^\theta}
\def\La{L_1^\theta}
\def\Ia{y}
\def\I{\mathds{1}}
\newacronym{loe}{LOE}{latent outlier exposure}
\newacronym{aloe}{SOEL}{\textbf{s}emi-supervised \textbf{o}utlier \textbf{e}xposure with a \textbf{l}imited labeling budget}
\newacronym{ntl}{NTL}{neural transformation learning}
\newacronym{mhrot}{MHRot}{multi-head RotNet}
\newacronym{ad}{AD}{anomaly detection}

\def\s{S}
\def\sau{s_1}%
\def\snu{s_0}%
\def\saq{\mu_1}%
\def\snq{\mu_0}%
\def\fz{f_z}
\def\unif{\text{Unif}}
\def\kmeans{k-means++ }
\newcommand{\ditto}[1][.4pt]{superv. (\Cref{eqn:loss})}
\def\Margin{\text{Mar}}
\def\HybridA{\text{Hybr1}}
\def\PositiveB{\text{Pos1}}
\def\PositiveA{\text{Pos2}}
\def\RandomA{\text{Rand1}}
\def\RandomB{\text{Rand2}}
\def\HybridB{\text{Hybr2}}
\def\HybridC{\text{Hybr3}}
\Crefname{figure}{Fig.}{Figs.}
\Crefname{table}{Tab.}{Tabs.}
\Crefname{section}{Sec.}{Secs.}
\Crefname{proposition}{Prop.}{Props.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{appendix}{Supp.}{Supps.}
\Crefname{theorem}{Thm.}{Thms.}
\Crefname{algorithm}{Alg.}{Algs.}

\newcommand{\sm}[1]{{\color{blue} \bf SM: #1}}
\newcommand{\mrr}[1]{{\color{green} \bf MR: #1}}


\usepackage{booktabs,array}
\def\Midrule{\midrule[\heavyrulewidth]}
\newcount\rowc

\def\ttabular{%
\hbox\bgroup
\let\\\cr
\def\rulea{\ifnum\rowc=\@ne \hrule height 1.3pt \fi}
\def\ruleb{
\ifnum\rowc=1\hrule height 1.3pt \else
\ifnum\rowc=6\hrule height \heavyrulewidth 
   \else \hrule height \lightrulewidth\fi\fi}
\valign\bgroup
\global\rowc\@ne
\rulea
\hbox to 10em{\strut \hfill##\hfill}%
\ruleb
&&%
\global\advance\rowc\@ne
\hbox to 10em{\strut\hfill##\hfill}%
\ruleb
\cr}
\def\endttabular{%
\crcr\egroup\egroup}


\newcommand{\al}[1]{{\color{blue} #1}}
\newcommand{\rbt}[1]{#1}





==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/math-commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\erf}{\mathrm{\,erf}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/abstract.tex <==
\begin{abstract}
Selecting informative data points for expert feedback can significantly improve the performance of \gls{ad} in various contexts, such as medical diagnostics or fraud detection. In this paper, we determine a set of theoretical conditions under which anomaly scores generalize from labeled queries to unlabeled data. Motivated by these results, we propose a data labeling strategy with optimal data coverage under labeling budget constraints. In addition, we propose a new learning framework for semi-supervised \gls{ad}. 
Extensive experiments on image, tabular, and video data sets show that our approach results in state-of-the-art semi-supervised \gls{ad} performance under labeling budget constraints.
\end{abstract}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/acknowledgement.tex <==
\section*{Acknowledgements}
SM acknowledges support by the National Science Foundation (NSF) under an NSF CAREER Award, award numbers 2003237 and 2007719, by the Department of Energy under grant DE-SC0022331, by the HPI Research Center in Machine Learning and Data Science at UC Irvine, by the IARPA WRIVA program, and by gifts from Qualcomm and Disney. Part of this work was conducted within the DFG research unit FOR 5359 on Deep Learning on Sparse Chemical Process Data. MK acknowledges support by the Carl-Zeiss Foundation, the DFG awards KL 2698/2-1, KL 2698/5-1, KL 2698/6-1, and KL 2698/7-1, and the BMBF awards 03|B0770E and 01|S21010C.

The Bosch Group is carbon neutral. Administration, manufacturing and research activities do no longer leave a carbon footprint. This also includes GPU clusters on which the experiments have been performed.

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:discussion}




We introduced semi-supervised outlier exposure with a limited labeling budget (\gls{aloe}). 
Inspired by a set of conditions that guarantee the generalization of anomaly score rankings from queried to unqueried data, we proposed to use a diversified querying strategy %
and a combination of two losses for queried and unqueried samples. By weighting the losses equally to each other and by estimating the unknown contamination rate from queried samples, we were able to make our approach free of its most important hyperparameters, making it easy to use. An extensive empirical study on images, tabular data, and video 
confirmed the efficacy of \gls{aloe} as a semi-supervised learning framework compatible with many existing losses for \gls{ad}.


\textbf{Limitations:} The success of our approach relies on several heuristics that we demonstrated were empirically effective but that cannot be proven rigorously. Estimation of the contamination ratio can be noisy when the query set is small---but the LOE loss is robust even under misspecification of the contamination ratio \citep{qiu2022latent}. The diversified sampling strategy becomes expensive when the dataset is large, but this can be mitigated by random data thinning.%

\textbf{Societal Impacts:} The use of human labels for anomaly detection runs the risk of introducing potential human biases in the definition of what is anomalous, particularly for datasets involving human subjects. Since our approach relies heavily on a relatively small number of human labels, the deployment of our approach with real human labelers would benefit by having guidelines for the labelers in terms of providing fair labels and avoiding amplification of bias.

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\input{tables/methods}
We study \gls{aloe} on standard image benchmarks, medical images, tabular data, and surveillance videos.
Our extensive empirical study establishes how our proposed method compares to eight \gls{ad} methods with labeling budgets implemented as baselines.
We first describe the baselines and their implementations (\Cref{tab:baselines}) and then the experiments on images (\Cref{sec:image_exp}), tabular data (\Cref{sec:tab_exp}), videos (\Cref{sec:video_exp}) and finally additional experiments (\Cref{sec:add-exp}). %

\input{tables/results}
\textbf{Baselines.} 
Most existing baselines apply their proposed querying and training strategies to shallow \gls{ad} methods or sub-optimal deep models (e.g., autoencoders \citep{zhou2017anomaly}).
In recent years, these approaches have consistently been outperformed by self-supervised \gls{ad} methods \citep{hendrycks2019using}. For a fair comparison, we endow all baselines with the same self-supervised backbone models also used in our method. %
By default we use \gls{ntl} \citep{qiu2021neural} as the backbone model, which was identified as state-of-the-art in a recent independent comparison of 13 models \citep{alvarez2022revealing}. Results with other backbone models are shown in \Cref{app:ablation_model}. %

The baselines are summarized in \Cref{tab:baselines} and detailed in \Cref{sec:baselines}.  
They differ in their querying strategies (col. 3) and training strategies (col. 4 \& 5): the unlabeled data is either ignored or modeled with a one-class objective. 
Most baselines incorporate the labeled data by a supervised loss (\Cref{eqn:loss}).
As an exception, \citet{ning2022deep} remove all queried anomalies and then train a weighted one-class objective on the remaining data. All baselines weigh the unsupervised and supervised losses equally. 
They differ in their querying strategies, summarized below:
\vspace{-7pt}
\begin{itemize}[leftmargin=*,itemsep=-2pt]
    \item {\bf Margin query} selects samples close to the boundary of the normality region deterministically. The method uses the true contamination ratio to choose an ideal boundary.
    \item {\bf Margin diverse query} combines margin query with neighborhood-based diversification. 
    It selects samples that are not $k$-nearest neighbors of the queried set.
    Thus samples are both diverse and close to the boundary.
    \item {\bf Most positive query} always selects the top-ranked samples ordered by their anomaly scores.
    \item {\bf Positive diverse query} combines querying according to anomaly scores with distance-based diversification. 
    The selection criterion combines anomaly score and the minimum Euclidean distance to all queried samples.
    \item {\bf Random query} draws samples uniformly.  
    \item {\bf Positive random query} samples uniformly among the top $50\%$ data ranked by anomaly scores.  
\end{itemize}
\vspace{-2pt}

\textbf{Implementation Details.}
In all experiments, we use a \gls{ntl} \citep{qiu2021neural} backbone model for all methods.  %
Experiments with other backbone models are shown in \Cref{app:ablation_model}.
On images and videos, \gls{ntl} is built upon the penultimate layer output of a frozen ResNet-152 pre-trained on ImageNet.
\gls{ntl} is trained for one epoch, after which all $|\gQ|$ queries are labeled at once. %
The contamination ratio $\alpha$ in \gls{aloe} is estimated immediately after the querying step and then fixed for the remaining training process. 
We follow \citet{qiu2022latent} and set $\tilde{y}_i = 0.5$ for inferred anomalies. This accounts for the uncertainty of whether the sample truly is an anomaly. More details are given in \Cref{sec:implementation} and \Cref{alg:aloe}.


\input{figures/image_data}
\subsection{Experiments on Image Data}
\label{sec:image_exp}
We study \gls{aloe} on standard image benchmarks to establish how it compares to eight well-known baselines with various querying and training strategies.
Informative querying plays an important role in medical domains where expert labeling is expensive. Hence, we also study nine medical datasets from \citet{medmnistv2}. 
We describe the datasets, the evaluation protocol, and finally the results of our study.


\textbf{Image Benchmarks.}
We experiment with two popular image benchmarks: CIFAR-10 and Fashion-MNIST. These have been widely used in previous papers on %
deep \gls{ad}  
\citep{ruff2018deep,golan2018deep,hendrycks2019using,bergman2020classification}. 


\textbf{Medical Images.}
Since medical imaging is an important practical application of \gls{ad}, we also study \gls{aloe} on medical images. The datasets we consider cover different data modalities (e.g., X-ray, CT, electron microscope) and their characteristic image features can be very different from natural images.   
Our empirical study includes all 2D image datasets presented in \citet{medmnistv2}
that have more than 500 samples in each class, including \rbt{Blood, OrganA, OrganC, OrganS, OCT, Pathology, Pneumonia, and Tissue.} 
We also include \rbt{Dermatoscope} but restricted to the classes with more than 500 training samples. %

\textbf{Evaluation Protocol.}
We follow the community standard known as the ``one-vs.-rest'' protocol to turn these classification datasets into a test-bed for \gls{ad} \citep{ruff2018deep,hendrycks2019using,bergman2020classification}.
While respecting the original train and test split of these datasets, the protocol iterates over the classes and treats each class in turn as normal. Random samples from the other classes are used to contaminate the data. The training set is then a mixture of unlabeled normal and abnormal samples with a contamination ratio of $10\%$ \citep{ruff2019deep,wang2019effective,qiu2022latent}. 
This protocol can simulate a ``human expert'' to provide labels for the queried samples because the datasets provide ground-truth class labels.
The reported results (in terms of AUC $\%$) for each dataset are averaged over the number of experiments (i.e., classes) and over five independent runs. %



 

\textbf{Results.}
We report the evaluation results of our method (\gls{aloe}) and the eight baselines on all eleven image datasets in \Cref{tab:img_results}. 
When querying 20 samples, our proposed method \gls{aloe} significantly outperforms the best-performing baseline by 6 percentage points on average across all datasets.
We also study detection performance as the query budget increases from $20$ to $160$ in \Cref{fig:img_data}. %
The results show that, with a small budget of 20 samples, \gls{aloe} (by querying diverse and informative samples) makes better usage of the labels than the other baselines and thus leads to better performance by a large margin. As more samples are queried, the performance of almost all methods increases but even for $160$ queries when the added benefit from adding more queries starts to saturate, \gls{aloe}  still outperforms the baselines.
\vspace{-0.5em}

\input{tables/tabular}
\subsection{Experiments on Tabular Data}
\label{sec:tab_exp}
Many practical use cases of \gls{ad} (e.g., in health care or cyber security) are concerned with tabular data.
For this reason, we study \gls{aloe} on four tabular datasets from various domains. We find that it outperforms existing baselines, even with as few as 10 queries. We also confirmed the fact that our deep models are competitive with classical methods for tabular data in \Cref{app:more-comp}.

\textbf{Tabular Datasets.} 
Our study includes the four multi-dimensional tabular datasets from the ODDS repository which have an outlier ratio of at least $30\%$. This is necessary to ensure that there are enough anomalies available to remove from the test set and add to the clean training set (which is randomly sub-sampled to half its size) to achieve a contamination ratio of $10\%$. The datasets are BreastW, Ionosphere, Pima, and Satellite. %
As in the image experiments, there is one round of querying, in which $10$ samples are labeled. For each dataset, we report the averaged F1-score (\%) with standard deviations over five runs with random train-test splits and random initialization. %

\textbf{Results.}
\gls{aloe} performs best on 3 of 4 datasets and outperforms all baselines by 3.2 percentage points on average. Diverse querying best utilizes the query budget to label the diverse and informative data points, yielding a consistent improvement over existing baselines on tabular data. 


\subsection{Experiments on Video Data}
\label{sec:video_exp}
\input{figures/video_data}

Detecting unusual objects in surveillance videos is an important application area for \gls{ad}. Due to the large variability in abnormal objects and suspicious behavior in surveillance videos, expert feedback is very valuable to train an anomaly detector in a semi-supervised manner. We use \gls{ntl} as the backbone model and  study \gls{aloe} on a public surveillance video dataset (UCSD Peds1). The goal is to detect abnormal video frames that contain non-pedestrian objects. %

Following \citet{pang2020self}, we subsample a mix of normal and abnormal frames for training (using an anomaly ratio of $0.3$) and use the remaining frames for testing.
Before running any of the methods, a ResNet pretrained on ImageNet is used to obtain a fixed feature vector for each frame. We vary the query budget from $|\gQ|=20$ to $|\gQ|=160$ and compare \gls{aloe} to all baselines. %
Results in terms of average AUC and standard error over five independent runs are reported in \Cref{fig:video_data}. \gls{aloe} consistently outperforms all baselines, especially for smaller querying budgets. %



\subsection{Additional Experiments}
\label{sec:add-exp}
In \Cref{app:ablation}, we provide additional experiments and ablations demonstrating \gls{aloe}'s strong performance and justifying modeling choices. The three most important findings are:
\vspace{-8pt}
\begin{itemize}[leftmargin=*,itemsep=-4pt]
\item {\bf \gls{aloe} vs. Active Learning:} Our framework is superior to its extension to the sequential active learning (\Cref{fig:img-data-seq}).
\item {\bf Varying Contamination Ratio:} \Cref{fig:robust-ratio} demonstrates that \gls{aloe} dominates under varying contamination ratios (1\%, 5\%, 20\%). In addition, \Cref{tab:alpha-estimate} confirms that \Cref{eq:alpha-is} reliably estimates 
 $\alpha$ on both CIFAR-10 and F-MNIST. 
\item {\bf Backbone Models:} \Cref{tab:backbone-dsvdd-mhrot} 
shows that \gls{aloe} also performs best for the backbone models  MHRot~\citep{hendrycks2019using} and DSVDD~\citep{ruff2018deep}.
\end{itemize}
\vspace{-8pt}
In addition, we provide an ablation of the temperature $\tau$ (\Cref{tab:ablation-tau}), a discussion on the effects of initialization randomness (\Cref{app:rand-init}), an ablation study of the pseudo-label $\tilde y$ values (\Cref{tab:ablation-pseudo-y}), a comparison to binary classification (\Cref{fig:img-data-bce}), an ablation of the \gls{aloe} loss components, an ablation of querying strategies (\Cref{fig:ablation-query}),
additional methods for inferring $y$  (\Cref{fig:semisuper-comparison}), and comparison to additional semi-supervised baselines (\Cref{fig:semisuper-comparison}, \Cref{tab:tab_knn}).





==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/introduction.tex <==
\section{Introduction}
Detecting anomalies in data is a fundamental task in machine learning with applications across multiple domains, from industrial fault detection to medical diagnosis. The main idea is to train a model (such as a neural network) on a data set of ``normal'' samples to minimize the loss of an auxiliary (e.g., self-supervised) task. Using the loss function to score test data, one hopes to obtain low scores for normal data and high scores for anomalies \citep{ruff2021unifying}. 

In practice, the training data is often contaminated with unlabeled anomalies that differ in unknown ways from the i.i.d. samples of normal data. 
No access to a binary anomaly label (indicating whether a sample is normal or not) makes learning the anomaly scoring function from contaminated data challenging; the training signal has to come exclusively from the input features (typically real-valued vectors).  Many approaches either assume that the unlabeled anomalies are too rarely encountered during training to affect learning \citep{wang2019effective} or try to detect and exploit the anomalies in the training data (e.g., \citet{qiu2022latent}).

While \gls{ad} is typically an unsupervised training task, sometimes expert feedback is available to check if individual samples are normal or not. For example, in a medical setting, one may ask a medical doctor to confirm whether a given image reflects normal or abnormal cellular tissue. Other application areas include detecting network intrusions or machine failures. Anomaly labels are usually expensive to obtain but are very valuable to guide an anomaly detector during training. For example, in \Cref{fig:toy-data}, we can see that our method, with only one labeled query (\Cref{fig:toy-data}~d) is almost on par with supervised \gls{ad} (\Cref{fig:toy-data}~a). However, the supervised setting is unrealistic, since expert feedback is typically expensive. Instead, it is essential to develop effective strategies for querying informative data points. 


Previous work on \gls{ad} under a labeling budget primarily involves domain-specific applications and/or ad hoc architectures, making it hard to disentangle modeling choices from querying strategies \citep{trittenbach2021overview}. 
In contrast, this paper theoretically and empirically studies generalization performance using various labeling budgets, querying strategies, and losses. 

In summary, our main contributions are as follows:
\vspace{-7pt} %
\begin{enumerate}[leftmargin=*,itemsep=-2pt]
\item We prove that the ranking of anomaly scores generalizes from labeled queries to unlabeled data under certain conditions that characterize how well the queries cover the data. Based on this theory, we propose a diverse querying strategy for deep \gls{ad} under labeling budget constraints.

\item We propose \gls{aloe}, a semi-supervised learning framework  compatible with a large number of deep \gls{ad} losses. 
We show how all major hyperparameters can be %
eliminated, making \gls{aloe} easy to use.
To this end, we provide an estimate for the anomaly ratio in the data. 

\item We provide an extensive benchmark for deep \gls{ad} with a limited labeling budget. %
Our experiments on image, tabular, and video data provide evidence that \gls{aloe} outperforms existing methods significantly. Comprehensive ablations disentangle the benefits of each component.


\end{enumerate}

Our paper is structured as follows. \Cref{sec:methods} introduces  the problem setting we address and our main algorithm. \Cref{sec:related} discusses related work in deep \gls{ad}. \Cref{sec:experiments} discusses experimental results on each of image, video, and tabular data. Finally, we conclude this work in Section \ref{sec:discussion}. 



==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/methods.tex <==
\input{figures/toy_example.tex}

\section{Methods}
\label{sec:methods}

\subsection{Notation and Problem Statement}%
\label{sec:prob-setup}
Consider a dataset $\{\vx_i\}_{i=1}^N$ where the datapoints $\vx_i$ are i.i.d. samples from a mixture distribution  $p(\vx)=(1-\alpha)p_0(\vx) + \alpha p_1(\vx)$. The distribution $p_0(\vx)$ corresponds to the normal data, while $p_1(\vx)$ corresponds to anomalous data. We assume that $0 \leq \alpha < 0.5$, i.e., that the anomalous data is non-dominant in the mixture; in practice, $\alpha \ll 0.5$. 

In the \gls{ad} problem, we wish to use the data to train an anomaly detector in the form of a parametric anomaly score function $\s(\vx;\theta)$. Once trained this score function is thresholded to determine whether a datapoint $\vx_i$ is anomalous, as indicated by the binary anomaly label  $y_i := y(\vx_i) \in \{0 := \text{``normal''}, 1:=\text{``abnormal''}\}$.

We focus on the situation where the training data is unlabeled (only $\vx_i$ is known, not $y_i$), but where we have access to an oracle (e.g., a human expert) that is able to provide labels $y_i$ for a budgeted number $K$ of the $N$ training points. 


 

\subsection{Outline of the Technical Approach}

Our work addresses the following questions: How to best select informative data points for labeling -- this is called the {\em querying strategy}, how to best learn an anomaly detector from both the labeled and unlabeled 
data in a semi-supervised fashion, and how to make the approach easy to use by eliminating a crucial hyper-parameter.

\textbf{Querying Strategy.} A successful approach for deep \gls{ad} under labeling budget constraints will require a strategy for selecting the most beneficial set of queries. We choose a theoretically-grounded approach based on generalization performance. For this, we exploit that at test-time an \gls{ad} method will threshold the anomaly scores to distinguish between normal samples and anomalies. This means that the quality of a scoring function is not determined by the absolute anomaly scores but only by their relative ranking. 
In \Cref{sec:active-learning}, we characterize a favorable property of the query set which can guarantee that the ranking of anomaly scores generalizes from the labeled data to unlabeled samples. Since this is desirable, we derive a querying strategy that under a limited labeling budget best fulfills the favorable properties put forth by our analysis. 


\textbf{Semi-supervised Outlier Exposure.} As a second contribution, we propose a semi-supervised learning framework that best exploits both the labeled query set and the unlabeled data. It builds on supervised \gls{ad} and \gls{loe} which we review in \Cref{sec:background}. 
We present \gls{aloe} in \Cref{sec:aloe-loss}. The \gls{aloe} training objective is designed to receive opposing training signals from the normal samples and the anomalies. An EM-style algorithm alternates between estimating the anomaly labels of the unlabaled data and improving the anomaly scoring function using the data samples and their given or estimated labels.

\textbf{Hyperparameter Elimination.} Like related methods discussed in \Cref{sec:related}, \gls{aloe} has an important hyperparameter $\alpha$ which corresponds to the expected fraction of anomalies in the data. While previous work has to assume that $\alpha$ is known \citep{qiu2022latent}, our proposed method presents an opportunity to estimate it. 
The estimate has to account for the fact that the optimal querying strategy derived from our theory in \Cref{sec:active-learning} is not i.i.d.. In \Cref{sec:alpha}, we provide an estimate of $\alpha$ for any stochastic querying strategy.


\subsection{Background: Deep \gls{ad}}
\label{sec:background}
In deep \gls{ad}, 
 auxiliary losses help learn the anomaly scoring function $\s(\vx;\theta)$. Popular losses include autoencoder-based losses \citep{zhou2017anomaly}, the deep SVDD loss \citep{ruff2018deep}, or the neural transformation learning loss \citep{qiu2021neural}. It is assumed that minimizing such a 
 loss $L^\theta_0(\vx)\equiv {\cal L}_0(\s(\vx;\theta))$  over ``normal'' data leads to a desirable scoring function that assigns low scores to normal samples and high scores to anomalies. 

Most deep \gls{ad} methods optimize such an objective over an entire unlabeled data set, even if it contains unknown anomalies. It is assumed that the anomalies are rare enough that they will not dilute the training signal provided by the normal samples ({\em inlier priority}, \citep{wang2019effective}). Building on the ideas of \citet{ruff2019deep} that synthetic anomalies can provide valuable training signal, \citet{qiu2022latent} show how to discover and exploit anomalies by treating the anomaly labels as latent variables in training.

The key idea of \citet{ruff2019deep} is to construct a complementary loss $L^\theta_1(\vx)\equiv {\cal L}_1(\s(\vx;\theta))$ for anomalies that has an opposing effect to the normal loss $L^\theta_0(\vx)$. For example, the deep SVDD loss $L_0^\theta(\vx)=||f_\theta(\vx)-{\bf c}||^2$, with feature extractor $f_\theta$, pulls normal data points towards a fixed center $c$ \citep{ruff2018deep}. The opposing loss for anomalies, defined in \citet{ruff2019deep} as $L_1^\theta(\vx) = 1/L_0^\theta(\vx)$, pushes abnormal data away from the center.

 





\textbf{Supervised \gls{ad}.} Using only the labeled data indexed by $\gQ$ one could train $\s(\vx;\theta)$ using a supervised loss \citep{hendrycks2018deep,gornitz2013toward}
\begin{equation}
\label{eqn:loss}
 {\cal L}_\gQ(\theta) = \frac{1}{|\gQ|}\sum_{j\in \gQ} \big(y_j \La(\vx_j) + (1-y_j) \Ln(\vx_j) \big) .
\end{equation}
\textbf{Latent Outlier Exposure.}
Latent outlier exposure (LOE, \citep{qiu2022latent}) is an unsupervised \gls{ad} framework that uses the same loss as \Cref{eqn:loss} but treats the labels $y$ as latent variables. An EM-style algorithm alternates between optimizing the model w.r.t. $\theta$ and inferring the labels $y$. 


In this work, we propose semi-supervised outlier exposure with a limited labeling budget (SOEL) which builds on these ideas. We next present the querying strategy and \rbt{when the querying strategy leads to correct ranking of anomaly scores (\Cref{sec:active-learning}),} the \gls{aloe} loss (\Cref{sec:aloe-loss}), and how the hyperparameter $\alpha$ can be eliminated (\Cref{sec:alpha})



\subsection{Querying Strategies for \gls{ad}} 
\label{sec:active-learning}

The first ingredient of \gls{aloe} is a querying strategy for selecting informative data points to be labeled,
which we derive from theoretical considerations. %
An important property of the querying strategy is how well it covers unlabeled data. The quality of a querying strategy is determined by the smallest radius $\delta$ such that all unlabeled points are within distance $\delta$ of one queried sample of the same type. In this paper, we prove that if the queries cover both the normal data and the anomalies well (i.e., if $\delta$ is small), a learned anomaly detector that satisfies certain conditions is guaranteed to generalize correctly to the unlabeled data (The exact statement and its conditions will be provided in \Cref{thm:rank}). Based on this insight, we propose to use a querying strategy that is better suited for deep \gls{ad} than previous work.

\input{thms/thm1-ranking}

In \Cref{app:thm1}, we prove \Cref{thm:rank} and discuss the assumptions. An implication of this theorem is that a smaller $\delta$ corresponding to a tighter cover of the data leads to better-generalized ranking performance. As detailed in \Cref{app:thm1}, there is a connection between correct anomaly score ranking and high AUROC performance, a common evaluation metric for \gls{ad}.

Existing methods use querying strategies that do not have good coverage and are therefore not optimal under \Cref{thm:rank}. For a limited querying budget, random querying puts too much weight on high-density areas of the data space, while other strategies only query locally, e.g., close to an estimated decision boundary between normal and abnormal data. 

\textbf{Proposed Querying Strategy.} Based on \Cref{thm:rank}, we propose a querying strategy that encourages tight coverage: diverse querying.
In practice, we use the seeding algorithm of \kmeans which is usually used to initialize diverse clusters.\footnote{This has complexity $O(KN)$ which can be reduced to $O(K\log N)$ using scalable alternatives \citep{bahmani2012scalable}.}  
It iteratively samples another data point to be added to the query set $\gQ$ until the labeling budget is reached. Given the existing queried samples, the probability of drawing another query from the unlabeled set $\gU$ is proportional to its distance to the closest sample already in the query set $\gQ$:
\begin{align}
\label{eq:query-prob}
    p_{\rm query} (\vx_i) = \softmax\big(h(\vx_i)/\tau\big) \quad \forall i \in \gU,
\end{align}
The temperature parameter $\tau$ controls the diversity of the sampling procedure, and  
$h(\vx_i) = \min_{\vx_j \in \mathcal{Q}} d(\vx_i,\vx_j)$ is the distance of a sample $\vx_i$ to the query set $\mathcal{Q}$.
For a meaningful notion of distance, we define $d$ in an embedding space as $d(\vx,\vx') = \|\phi(\vx)-\phi(\vx')\|_2$, where $\phi$ is a neural feature map. We stress that all deep methods considered in this paper have an associated feature map that we can use.
The fact that L2 distance is used in the querying strategy is not an ad-hoc choice but rather aligned with the $\delta$-ball radius definition (\Cref{eq:delta-est} in \Cref{app:thm1}) in \Cref{thm:rank}. 

In \Cref{app:thm1}, we discuss the cover radius and empirically validate that diverse querying leads to smaller $\delta$ than others and is hence advantageous for \gls{ad}.

\subsection{Semi-supervised Outlier Exposure Loss (SOEL)}
\label{sec:aloe-loss}

We next consider how to use both labeled and unlabeled samples in training. We propose \gls{aloe} whose loss combines the unsupervised \gls{ad} loss of LOE~\citep{qiu2022latent} for the unlabeled data with the supervised loss (\Cref{eqn:loss}) for the labeled samples. 
For all queried data (with index set $\gQ$), we assume that ground truth labels $y_i$  are available, while for unqueried data (with index set $\gU$), the labels $\tilde{y}_i$ are unknown. Adding both losses together yields
\begin{align}
\label{eqn:loss-2}
 {\cal L}(\theta, \tilde{\vy}) = \frac{1}{|\gQ|}\sum_{j\in \gQ} \big(y_j \La(\vx_j) + (1-y_j) \Ln(\vx_j) \big) + \nonumber \\ 
 \frac{1}{|\gU|}\sum_{i\in \gU} \big(\tilde{y}_i \La(\vx_i) + (1-\tilde{y}_i) \Ln(\vx_i)\big).
\end{align}
Similar to \citet{qiu2022latent}, optimizing this loss involves a block coordinate ascent scheme that alternates between inferring the unknown labels and taking gradient steps to minimize \Cref{eqn:loss-2} with the inferred labels. In each iteration, the pseudo labels $\tilde{y}_i$ for $i\in \gU$ are obtained by minimizing \Cref{eqn:loss-2} subject to a constraint of $\sum_{i\in\gQ} y_i + \sum_{i\in\gU} \tilde{y}_i = \alpha N$.     
The constraint ensures that the inferred anomaly labels respect a certain contamination ratio $\alpha$. To be specific, let $\tilde\alpha$ denote the fraction of anomalies among the \emph{unqueried} set $\gU$, so that 
$\tilde\alpha |\gU| + \sum_{j\in\gQ}y_j =\alpha N$. 
The constrained optimization problem is then solved by using the current anomaly score function $S$ to rank the unlabeled samples and assign the top $\tilde\alpha$-quantile of the associated labels $\tilde y_i$ to the value $1$, and the remaining to the value $0$. 

We illustrate \gls{aloe}'s effect on a 2D toy data example in \Cref{fig:toy-data}, where \gls{aloe} (\textbf{d}) almost achieves the same performance as the supervised AD (\textbf{c}) with only one queried point.   %


In theory, $\alpha$ could be treated as a hyperparameter, but eliminating hyperparameters is important in \gls{ad}. In many practical applications of \gls{ad}, there is no labeled data that can be used for validation. While \citet{qiu2022latent} have to assume that the contamination ratio is given, \gls{aloe} provides an opportunity to estimate $\alpha$. In \Cref{sec:alpha}, we develop an importance-sampling based approach to estimate $\alpha$ from the labeled data. \rbt{Estimating this ratio can be beneficial for many \gls{ad} algorithms, including OC-SVM~\citep{scholkopf2001estimating}, kNN~\citep{ramaswamy2000efficient}, Robust PCA/Auto-encoder~\citep{zhou2017anomaly}, and Soft-boundary deep SVDD~\citep{ruff2018deep}. When working with contaminated data, these algorithms require a decent estimate of the contamination ratio for good performance.} %


Another noteworthy aspect of the \gls{aloe} loss is that it weighs the \emph{averaged} losses equally to each other. In \Cref{app:ablation_weight}, we empirically show that equal weighting yields the best results among a large range of various weights. This provides more weight to every queried data point than to an unqueried one, because we expect the labeled samples to be more informative. On the other hand, it ensures that neither loss component will dominate the learning task. Our equal weighting scheme is also practical because it avoids a hyperparameter.







\subsection{Contamination Ratio Estimation.}
\label{sec:alpha}
To eliminate a critical hyperparameter in our approach, we estimate the \emph{contamination ratio} $\alpha$, i.e., the fraction of anomalies in the dataset.  Under a few assumptions, we show how to estimate this parameter using mini-batches composed of on non-i.i.d. samples. 

We consider the contamination ratio $\alpha$ as the fraction of anomalies in the data. We draw on the notation from~\Cref{sec:prob-setup} to define $\Ia(\vx)$ as an oracle, outputting $1$ if $\vx$ is an anomaly, and $0$ otherwise (e.g., upon \emph{querying} $\vx$). We can now write $\alpha = \mathbb{E}_{p(\vx)} [\Ia(\vx)]$. 

Estimating $\alpha$ would be trivial given an unlimited querying budget of i.i.d. data samples. The difficulty arises due to the fact that (1) our querying budget is limited, and (2) we query data in a non-i.i.d. fashion so that the sample average is not representative of the anomaly ratio of the full data set. 

Since the queried data points are not independently sampled, we cannot straightforwardly estimate $\alpha$ based on the empirical frequency of anomalies in the query $\gQ$. More precisely, our querying procedure results in a  chain of indices $\gQ = \{i_1, i_2, ..., i_{|\gQ|}\}$, where $i_1 \sim \rm{Unif}(1:N)$, and each conditional distribution $ i_k|i_{<k}$ is defined by \Cref{eq:query-prob}. We will show as follows that this sampling bias can be compensated using importance weights. 
 
As follows, we first propose an importance-weighted estimator of $\alpha$ and then prove the estimator is unbiased under certain idealized conditions specified by two assumptions about our querying strategy. Justifications for the two assumptions will be provided below.

For a random query $\gQ$, its anomaly scores $\{S(\vx_i): i\in\gQ\}$ and anomaly labels $\{\Ia(\vx_i):i\in\gQ\}$ are known. Write $S(\vx_i)$ as $s_i$ and let $p_s(s_i)$ denote the marginal density of population anomaly scores and $q_s(s_i)$ denote the marginal density of the queried samples' anomaly scores. Our importance-weighted estimator of the contamination ratio is
\begin{align}
\label{eq:alpha-is}
    \hat{\alpha} 
    = \frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia(\vx_i). 
\end{align}
As discussed above, $\Ia(\vx_i)$ are the ground truth anomaly labels, obtained from querying $\gQ$. The estimator takes into account that, upon repulsive sampling, we will sample data points in the tail regions of the data distribution more often than we would upon uniform sampling. 

In practice, we learn $p_s$ and $q_s$ using a kernel density estimator in the one-dimensional space of anomaly scores of the training data and the queried data, respectively. We set the bandwidth to the average spacing of scores. With the following two assumptions, \Cref{eq:alpha-is} is unbiased.

\textbf{Assumption 1.} \textsl{The anomaly scores $\{S(\vx_i): i \in \gQ\}$ in a query set $\gQ$ are approximately independently distributed.
}

\textbf{Assumption 2.} \textsl{
Let $\Ia_s(S(\vx))$ denote an oracle that assigns ground truth anomaly labels based on the model's anomaly scores $S(\vx)$.
We assume that such an oracle exists, i.e., the anomaly score $S(\vx)$ is a sufficient statistic of the ground truth anomaly labeling function: $\Ia_s(S(\vx)) = \Ia(\vx)$.}



Assumptions 1 and 2 are only approximations of reality. In our experiment section, we will show that they are good working assumptions to estimate anomaly ratios. Below, we will provide additional strong evidence that assumptions 1 and 2 are well justified. 

The following theorem is a consequence of them:




\input{thms/thm2-alpha}

\rbt{The proof is in \Cref{sec:assum-veri}.} 
\Cref{thm:alpha} allows us to estimate the contamination ratio based on a non-iid query set $\gQ$. 





\textbf{Discussion.} We empirically verified the fact that \Cref{thm:alpha} results in reliable estimates for varying contamination ratios 
in \Cref{app:alpha-est}. Since Assumptions 1 and 2 seem strong, we discuss their justifications and empirical validity next. 

While verifying the independence assumption (Assumption 1) rigorously is difficult, we tested for linear correlations between the scores (\Cref{sec:assum-veri-1}). We found that the absolute off-diagonal coefficient values are significantly smaller than one on CIFAR-10, providing support for Assumption 1. 
A heuristic argument can be provided to support the validity of Assumption 1 based on the following intuition. When data points are sampled diversely in a high-dimensional space, the negative correlations induced by their repulsive nature tend to diminish when the data is projected onto a one-dimensional subspace. This intuition stems from the fact that a high-dimensional ambient space offers ample dimensions for the data points to avoid clustering. To illustrate this, consider the scenario of sampling diverse locations on the Earth's surface, with each location representing a point in the high-dimensional space. By including points from various continents, we ensure diversity in their spatial distribution. However, when focusing solely on the altitude of these locations (such as distinguishing between mountain tops and flat land), it is plausible that the altitude levels are completely uncorrelated. While this heuristic argument provides an intuitive understanding, it is important to note that it does not offer a rigorous mathematical proof.

To test Assumption 2, we tested the degree to which the anomaly score is a sufficient statistic for anomaly scoring on the training set. The assumption would be violated if we could find pairs of training data $\vx_i$ and $\vx_j$, where $\vx_i\neq\vx_j$, with identical anomaly scores $S(\vx_i)=S(\vx_j)$ but different anomaly labels $\Ia_s(s_i)\neq \Ia_s(s_j)$\footnote{The condition $S(\vx_i)\neq S(\vx_j)$ for $\vx_i\neq\vx_j$ hints we can assign a unique label to each data point based on their scores.}. On FMNIST, we found 38 data pairs with matching scores, and none of them had opposite anomaly labels. For CIFAR-10, the numbers were 21 and 3, respectively. See \Cref{sec:assum-veri-3} for details. 







==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/sections/related-work.tex <==
\section{Related Work}
\label{sec:related}

\textbf{Deep Anomaly Detection.}
Many recent advances in anomaly detection are in the area of deep learning \citep{ruff2021unifying}. One early strategy was to use autoencoder- \citep{principi2017acoustic,zhou2017anomaly} or density-based models \citep{schlegl2017unsupervised, deecke2018image}. Another pioneering stream of research combines one-class classification \citep{scholkopf2001estimating} with deep learning for unsupervised \citep{ruff2018deep,ijcai2022p305} and semi-supervised \citep{ruff2019deep} anomaly detection. Many other approaches to deep anomaly detection are self-supervised. %
They employ a self-supervised loss function to train the detector and score anomalies \citep{golan2018deep,hendrycks2019using,bergman2020classification,qiu2021neural,shenkar2022anomaly,schneider2022detecting}. Our work resides in the self-supervised anomaly detection category and can be extended to other data modalities if an appropriate loss is provided.%

While all these methods assume that the training data consists of only normal samples, in many practical applications, the training pool may be contaminated with unidentified anomalies \citep{vilhjalmsson2013nature,poisoning1}.
This can be problematic because the detection accuracy typically deteriorates when the contamination ratio increases \citep{wang2019effective}. Addressing this, refinement \citep{zhou2017anomaly,yoon2021self} attempts to cleanse the training pool by removing anomalies therein, although they may provide valuable training signals. As a remedy, \citet{qiu2022latent} propose to jointly infer binary labels to each datum (normal vs. anomalous) while updating the model parameters based on outlier exposure. Our work also makes the contaminated data assumption and employs the training signal of abnormal data.

\textbf{Querying Strategies for Anomaly Detection.} Querying strategies play an important role in batch active learning \citep{sener2018active, ash2020deep, citovsky2021batch, pinsler2019bayesian, hoi2006large} but are less studied for anomaly detection.
The human-in-the-loop setup for anomaly detection has been pioneered by \citet{pelleg2004active}. %
Query samples are typically chosen locally, e.g., close to the decision boundary of a one-class SVM \citep{gornitz2013toward,yin2018active} or sampled according to a density model \citep{ghasemi2011active}. \citet{siddiqui2018feedback,das2016incorporating} propose to query the most anomalous instance, while \citet{das2019active} employ a tree-based ensemble to query both anomalous and diverse samples. A recent survey compares various aforementioned query strategies with one-class classifiers \citep{trittenbach2021overview}.

\citet{pimentel2020deep} query samples with the top anomaly scores for autoencoder-based methods, while \citet{ning2022deep} improve the querying by considering the diversity. \citet{tang2020deep} use an ensemble of deep anomaly detectors and query the most likely anomalies for each detector separately. \citet{russo2020active} query samples where the model is uncertain about the predictions. \citet{pang2021toward} and \citet{zha2020meta} propose querying strategies based on reinforcement learning, which requires labeled datasets. 

All these querying strategies do not optimize coverage as defined in \Cref{thm:rank}, and as a result, their generalization guarantees are less favorable than our method.   
Most querying strategies from the papers discussed above are fairly general and can be applied in combination with various backbone models. 
Since more powerful backbone models have been released since these earlier publications, we ensure a fair comparison by studying all querying strategies in combination with the same backbone models as \gls{aloe}.







==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/ablation-backbone.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{$|\gQ|=20$. AUC ($\%$) with standard deviation for anomaly detection on CIFAR-10 and F-MNIST. For all experiments, we set the contamination ratio as $10\%$. \gls{aloe} mitigates the performance drop when \gls{ntl} and \gls{mhrot} trained on the contaminated datasets. Results of the unsupervised method LOE are borrowed from \citet{qiu2022latent}.}
	\label{tab:ablation-backbone}
	\small
	\centering
	\vspace{1pt}
	
	\begin{tabular}{l@{\hskip 0.3in}cccc@{\hskip 0.3in}ccc}
        \toprule
        & \multicolumn{3}{c}{NTL} & & 
        \multicolumn{3}{c}{MHRot} \\
        \cmidrule(r){2-4} \cmidrule(r){6-8}
        & LOE & \kmeans & \gls{aloe} & & LOE & \kmeans & \gls{aloe} \\
		\cmidrule(r){2-4} \cmidrule(r){6-8}
		CIFAR-10 & 94.9$\pm$0.1 &95.6$\pm$0.3 &\textbf{96.3$\pm$0.3}& &86.3$\pm$0.2 &64.0$\pm$0.2 &\textbf{86.9$\pm$0.7}  \\ 
		F-MNIST &92.5$\pm$0.1 &94.3$\pm$0.2 &\textbf{94.8$\pm$0.4}& &91.2$\pm$0.4 &91.5$\pm$0.1 &\textbf{92.6$\pm$0.1} \\
        \bottomrule
	\end{tabular}
	
\end{table}




==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/ablation-pseudo-y.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{Performance of ablation study on $\tilde y$. AUROC (\%) on CIFAR-10 and F-MNIST when $|\gQ|=20$, the ground-truth contamination ratio is 0.1, and the backbone model is NTL. } %
	\label{tab:ablation-pseudo-y}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lcccccc}
        \toprule
		$\tilde y$ & 1.0 &0.875  &0.75 &0.625 &0.5 &0.25   \\
		\midrule
		CIFAR-10 &95.3 $\pm$ 0.6  &95.7 $\pm$ 0.4  &95.8 $\pm$ 0.4 &96.0 $\pm$ 0.5 &96.3 $\pm$ 0.3 &94.5 $\pm$ 0.3  \\
		F-MNIST & 94.5  $\pm$ 0.5  &94.5 $\pm$ 0.4  &94.6 $\pm$ 0.4 &94.6 $\pm$ 0.3 &94.8 $\pm$ 0.6 &94.0 $\pm$ 0.4\\
        \bottomrule
	\end{tabular}
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/ablation-tau.tex <==
\begin{table}[ht]
\vspace{-5pt}
	\caption{Performance of ablation study on $\tau$. AUROCs (\%) on CIFAR-10 and F-MNIST when $|\gQ|=20$, the ground-truth contamination ratio is 0.1, and the backbone model is NTL. } %
	\label{tab:ablation-tau}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lcccc}
        \toprule
		   $\tau$  & 1 & 0.1 & 0.01 & 0.001  \\
		\midrule
		CIFAR-10 &$93.2 \pm 1.7$  & $94.5 \pm 0.8$  & $96.3 \pm 0.3$ & $95.9 \pm 0.4$  \\
		F-MNIST & $91.8 \pm 1.4$ & $92.7 \pm 1.1$ & $94.8 \pm 0.6$ & $94.9 \pm 0.2$ \\
        \bottomrule
	\end{tabular}
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/contamination-ratio.tex <==



\begin{table}[ht]
\vspace{-5pt}
	\caption{Estimated contamination ratios on CIFAR-10 and F-MNIST when $|\gQ|=40$ and the backbone model is NTL. The first row shows the true contamination ratio ranging from $1\%$ to $45\%$. The estimations are repeated 50 times.} %
	\label{tab:alpha-estimate}
	\small
	\centering
	\vspace{1pt}
	\begin{tabular}{lccccc}
        \toprule
		     & 1\% & 5\% & 10\% & 15\% &20\% \\
		\midrule
		CIFAR-10 &$0.5\% \pm 1.2\%$ & $6.0\% \pm 3.3\%$ & $12.0\% \pm 4.4\%$ & $15.3\% \pm 4.5\%$ 
        & 18.9\% $\pm$ 5.4\%\\
		F-MNIST &$1.0\% \pm 1.5\%$ & $3.8\% \pm 2.3\%$ &  $8.7\% \pm 4.1\%$ & $12.8\% \pm 5.3\%$ 
        & 19.3\% $\pm$ 5.1\%\\
        \bottomrule
	\end{tabular}

        \begin{tabular}{lccccc}
        \toprule
		     &25\% &30\% &35\% &40\% &45\% \\
		\midrule
		CIFAR-10 &26.2\% $\pm$ 6.0\%   & 30.6\% $\pm$ 5.5\% &35.8\% $\pm$ 6.9\%  &42.0\% $\pm$ 7.7\%  &47.2\% $\pm$ 6.7\%\\
		F-MNIST &27.9\% $\pm$ 6.4\%  &31.8\% $\pm$ 6.1\% &38.3\% $\pm$ 6.5\% &43.1\% $\pm$ 5.7\% &48.9\% $\pm$ 5.6\% \\
        \bottomrule
	\end{tabular}
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/dsvdd-mhrot-image.tex <==
\begin{table}[ht]
	\caption{$|\gQ|=20$. AUC ($\%$) with standard deviation for anomaly detection on six datasets (CIFAR-10, F-MNIST, Blood, OrganA, OrganC, OrganS). The backbone models are \gls{mhrot}~\citep{hendrycks2019using} and Deep SVDD~\citep{ruff2018deep}. For all experiments, we set the contamination ratio as $10\%$. \gls{aloe} consistently outperforms two best-performing baselines on all six datasets.}
	\label{tab:backbone-dsvdd-mhrot}
	\small
	\centering
	\vspace{1pt}
	
	\begin{tabular}{l@{\hskip 0.3in}cccc@{\hskip 0.3in}ccc}
        \toprule
        & \multicolumn{3}{c}{MHRot} & & 
        \multicolumn{3}{c}{Deep SVDD} \\
        \cmidrule(r){2-4} \cmidrule(r){6-8}
        & \gls{aloe} & \HybridA & \HybridB & & \gls{aloe} & \HybridA & \HybridB \\
		\cmidrule(r){2-4} \cmidrule(r){6-8}
		CIFAR-10 & \textbf{86.9$\pm$0.7} & 83.9$\pm$0.1 & 49.1$\pm$2.0 && \bf93.1$\pm$0.2 & 89.0$\pm$0.6 & 91.3$\pm$1.0 \\ 
		F-MNIST &\textbf{92.6$\pm$0.1} & 87.1$\pm$0.2 & 58.9$\pm$5.7 && \bf91.4$\pm$0.5 & 90.9$\pm$0.4 & 82.5$\pm$2.9\\
        Blood &\textbf{83.3$\pm$0.2} & 81.1$\pm$2.5 & 61.8$\pm$2.1 && \bf80.2$\pm$1.1 & 79.7$\pm$1.2 & 77.2$\pm$3.0\\
        OrganA & \textbf{96.5$\pm$0.3} & 94.1$\pm$0.3 & 61.1$\pm$4.8 && \bf89.5$\pm$0.3 & 87.1$\pm$0.7 & 71.3$\pm$3.8\\
        OrganC & \textbf{92.1$\pm$0.2} & 91.6$\pm$0.1 & 70.9$\pm$0.8  && \bf87.5$\pm$0.7 & 85.3$\pm$0.8 & 84.2$\pm$0.9\\
        OrganS & \textbf{89.3$\pm$0.2} & 88.3$\pm$0.3 & 68.2$\pm$0.1  && \bf85.5$\pm$0.7 & 83.4$\pm$0.3 & 81.2$\pm$1.3\\
        \bottomrule
	\end{tabular}
	
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/hyperparameters.tex <==
\begin{table}[ht]
    \centering
    \small
    \begin{tabular}{ll|cccc}
    \toprule
    Model & Dataset &  Learning Rate & Epoch & Minibatch Size & $\tau$\\
    \midrule
    \multirow{5}{*}{NTL} & CIFAR-10 &  1e-4 & 30 & 512 & 1e-2 \\
        & F-MNIST &  1e-4 & 30 & 512 & 1e-2 \\
        & MedMNIST & 1e-4 & 30 & 512 & 1e-2 \\
        & ODDS & 1e-3 & 100 & $\lceil N/5 \rceil$ & 1e-2 \\
        & UCSD Peds1 & 1e-4 & 3$^*$ & 192 & 1e-2 \\
    \midrule
    \multirow{3}{*}{MHRot} & CIFAR-10 &  1e-3 & 15 & 10 & N/A \\
        & F-MNIST &  1e-4 & 15$^{**}$ & 10 & N/A \\
        & MedMNIST &  1e-4 & 15 & 10 & N/A \\
    \midrule
    \multirow{3}{*}{Deep SVDD} & CIFAR-10 & 1e-4 & 30 & 512 & 1e-2  \\
        & F-MNIST  & 1e-4 & 30 & 512 & 1e-2\\
        & MedMNIST & 1e-4 & 30 & 512 & 1e-2 \\
    \bottomrule
    \multicolumn{5}{l}{{\small $^*$\HybridB, \HybridC, \PositiveB, and \PositiveA~train 30 epochs. All other methods train 3 epochs.}}\\
    \multicolumn{5}{l}{{\small $^{**}$\gls{aloe} train 3 epochs. }}
    \end{tabular}
    \caption{A summary of optimization parameters for all methods.}
    \label{tab:opt-param}
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/knn-comparison.tex <==
\begin{table}[ht]
\vspace{-5pt}
    \caption{Comparisons with kNN method. We reported the F1-score ($\%$) with standard error for anomaly detection on tabular datasets when the query budget $K=10$. \gls{aloe} outperforms the kNN baseline. }
\label{tab:tab_knn}
    \centering
    \small
  \begin{tabular}{l|cc}
  \toprule
     & \bfseries $k^{\text{th}}$NN & \bfseries ALOE \\ 
  \midrule
\bfseries  BreastW  & 92.5$\pm$2.1	& \textbf{93.9$\pm$0.5}	\\ 
\bfseries Ionosphere & 88.1$\pm$1.3	& \textbf{91.8$\pm$1.1}	\\ 
 \bfseries Pima & 40.5$\pm$4.7	& \textbf{55.5$\pm$1.2}	\\ 
 \bfseries Satellite & 61.1$\pm$2.2	& \textbf{71.1$\pm$1.7}	\\ 
\midrule
\bfseries Average & 70.6 & \textbf{78.1} \\
  \bottomrule 
  \end{tabular}
 \vspace{-5pt}
\end{table}


==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/methods.tex <==

\begin{table*}[t!]
\vspace{-5pt}
	\caption{A summary of all compared experimental methods' query strategy and training strategy irrespective of their backbone models.}
	\label{tab:baselines}
 	\footnotesize
	\centering
	\begin{tabular}{lll@{\hskip 0.2in}cc}
        \toprule
		Name & Reference & Querying Strategy & Loss (labeled) & Loss (unlabeled)  \\
		\midrule
		\Margin & \citet{gornitz2013toward}  &margin query %
		& superv. (\Cref{eqn:loss}) & one class \\
        \HybridA & \citet{gornitz2013toward} & margin diverse query %
        & \ditto & one class  \\
        \PositiveB & \citet{pimentel2020deep} & most positive query & \ditto & none \\
        \PositiveA & \citet{barnabe2015active} & most positive query & \ditto & one class \\
        
        \RandomA & \citet{ruff2019deep} & random query & \ditto & one class  \\
        \RandomB & \citet{trittenbach2021overview} & positive random query & \ditto & one class    \\
        \HybridB &\citet{das2019active} &positive diverse query & \ditto & none \\
        \HybridC & \citet{ning2022deep} &positive diverse query & refinement & weighted one class \\
        \midrule
        SOEL& [ours] & diverse (\Cref{eq:query-prob}) & \multicolumn{2}{c}{ semi-supervised outlier exposure loss (\Cref{eqn:loss-2})} \\
        \bottomrule
	\end{tabular}
 	\vspace{-5pt}
\end{table*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/results.tex <==





\begin{table*}[t!]
\vspace{-5pt}
    \caption{AUC ($\%$) with standard deviation for anomaly detection on 11 image datasets when the query budget $|\gQ|=20$. \gls{aloe} outperforms all baselines by a large margin by querying diverse and informative samples.}%
\label{tab:img_results}
    \footnotesize
    \centering
  \begin{tabular}{l|ccccccccc}
  \toprule
     & \bfseries\Margin & \bfseries\HybridA & \bfseries\PositiveB & \bfseries\PositiveA & \bfseries\RandomA & \bfseries\RandomB & \bfseries\HybridB & \bfseries\HybridC & \bfseries SOEL \\ 
  \midrule
    \bfseries CIFAR10                  & 92.4$\pm$0.7                                    & 92.0$\pm$0.7                                     & 93.4$\pm$0.5                                       & 92.1$\pm$0.7                                       & 89.2$\pm$3.2                                     & 91.4$\pm$1.0                                     & 85.1$\pm$2.2                                     & 71.8$\pm$7.4                                     & \textbf{96.3$\pm$0.3}                  \\ 
\bfseries FMNIST                   & 93.1$\pm$0.4                                    & 92.6$\pm$0.4                                     & 92.2$\pm$0.6                                       & 89.3$\pm$1.0                                       & 84.0$\pm$3.8                                     & 90.6$\pm$1.1                                     & 88.7$\pm$1.4                                     & 82.6$\pm$4.3                                     & \textbf{94.8$\pm$0.6}                  \\ 
\bfseries Blood                    & 68.6$\pm$1.8                                    & 69.1$\pm$1.3                                     & 69.6$\pm$1.8                                       & 72.2$\pm$4.9                                       & 70.6$\pm$1.6                                     & 69.2$\pm$1.7                                     & 72.2$\pm$2.7                                     & 58.3$\pm$5.2                                     & \textbf{80.5$\pm$0.5}                  \\ 
\bfseries OrganA                   & 86.4$\pm$1.3                                    & 87.4$\pm$0.7                                     & 81.7$\pm$2.9                                       & 81.8$\pm$2.1                                       & 82.9$\pm$0.6                                     & 86.5$\pm$0.7                                     & 88.6$\pm$1.5                                     & 68.8$\pm$3.1                                     & \textbf{90.7$\pm$0.7}                  \\ 
\bfseries OrganC                   & 86.5$\pm$0.9                                    & 87.0$\pm$0.7                                     & 84.6$\pm$1.9                                       & 79.6$\pm$2.0                                       & 85.5$\pm$0.9                                     & 86.4$\pm$0.8                                     & 84.8$\pm$1.2                                     & 68.9$\pm$3.0                                     & \textbf{89.7$\pm$0.7}                  \\ 
\bfseries OrganS                   & 83.5$\pm$1.1                                    & 84.1$\pm$0.4                                     & 83.2$\pm$1.3                                       & 78.6$\pm$1.0                                       & 82.2$\pm$1.4                                     & 83.8$\pm$0.4                                     & 82.3$\pm$0.7                                     & 66.9$\pm$4.3                                     & \textbf{87.4$\pm$0.8}                  \\ 
\bfseries OCT                      & 64.4$\pm$3.7                                    & 63.3$\pm$1.8                                     & 63.8$\pm$4.4                                       & 63.0$\pm$4.0                                       & 59.7$\pm$1.9                                     & 62.1$\pm$4.3                                     & 63.0$\pm$7.6                                     & 56.2$\pm$4.5                                     & \textbf{68.5$\pm$3.4}                  \\ 
\bfseries Path                     & 82.7$\pm$2.4                                    & 86.0$\pm$1.1                                     & 77.5$\pm$2.0                                       & 80.2$\pm$3.5                                       & 83.2$\pm$1.6                                     & 83.9$\pm$2.9                                     & 86.1$\pm$2.0                                     & 75.1$\pm$4.2                                     & \textbf{88.1$\pm$1.1}                  \\ 
\bfseries Pneumonia                & 72.1$\pm$7.0                                    & 75.1$\pm$5.3                                     & 75.5$\pm$8.8                                       & 83.6$\pm$6.1                                       & 68.1$\pm$5.9                                     & 76.0$\pm$8.0                                     & 88.4$\pm$3.3                                     & 63.4$\pm$17.7                                    & \textbf{91.2$\pm$1.4}                  \\ 
\bfseries Tissue                   & 60.2$\pm$1.5                                    & 61.3$\pm$1.7                                     & 65.8$\pm$1.7                                       & 63.5$\pm$2.0                                       & 59.9$\pm$1.7                                     & 59.5$\pm$1.3                                     & 62.1$\pm$1.7                                     & 50.8$\pm$1.6                                     & \textbf{66.4$\pm$1.4}                  \\ 
\bfseries Derma                    & 62.6$\pm$3.8                                    & 63.1$\pm$4.7                                     & 66.6$\pm$2.3                                       & 66.4$\pm$4.3                                       & 64.5$\pm$4.8                                     & 68.3$\pm$2.1                                     & 57.2$\pm$13.3                                    & 48.0$\pm$13.6                                    & \textbf{73.5$\pm$2.5}                  \\ 
\midrule
\bfseries Average & 77.5 & 78.3 &  77.3  & 77.6 &75.4 &78.0 &78.0 &64.6 &\textbf{84.3} \\
  \bottomrule 
  \end{tabular}
 
\vspace{-5pt}
\end{table*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/tabular.tex <==






\begin{table*}[t!]
\vspace{-5pt}
    \caption{F1-score ($\%$) with standard deviation for anomaly detection on tabular data when the query budget $|\gQ|=10$. \gls{aloe} performs the best on 3 of 4 datasets and outperforms all baselines by 3.2 percentage points on average.}%
\label{tab:tab_results}
    \footnotesize
    \centering
  \begin{tabular}{l|ccccccccc}
  \toprule
     & \bfseries\Margin & \bfseries\HybridA & \bfseries\PositiveB & \bfseries\PositiveA & \bfseries\RandomA & \bfseries\RandomB & \bfseries\HybridB & \bfseries\HybridC & \bfseries \gls{aloe} \\ 
  \midrule
\bfseries  BreastW  & 81.6$\pm$0.7	& 83.3$\pm$2.0	& 58.6$\pm$7.7	& 81.3$\pm$0.8	& 87.1$\pm$1.0	& 82.9$\pm$1.1	& 55.0$\pm$6.0	& 79.6$\pm$4.9	& \textbf{93.9$\pm$0.5}	\\ 
\bfseries Ionosphere & 91.9$\pm$0.3	& \textbf{92.3$\pm$0.5}	& 56.1$\pm$6.2	& 91.1$\pm$0.8	& 91.1$\pm$0.3	& 91.9$\pm$0.6	& 64.0$\pm$4.6	& 88.2$\pm$0.9	& 91.8$\pm$1.1	\\ 
 \bfseries Pima & 50.1$\pm$1.3	& 49.2$\pm$1.9	& 48.5$\pm$0.4	& 52.4$\pm$0.8	& 53.6$\pm$1.1	& 51.9$\pm$2.0	& 53.8$\pm$4.0	& 48.4$\pm$0.7	& \textbf{55.5$\pm$1.2}	\\ 
 \bfseries Satellite & 64.2$\pm$1.2	& 66.2$\pm$1.7	& 57.0$\pm$3.0	& 56.7$\pm$3.2	& 67.7$\pm$1.2	& 66.6$\pm$0.8	& 48.6$\pm$6.9	& 56.9$\pm$7.0	& \textbf{71.1$\pm$1.7}	\\ 
\midrule
\bfseries Average & 72.0 & 72.8 & 55.1 & 70.4 & 74.9 & 73.3 & 55.4 &  68.3 & \textbf{78.1} \\
  \bottomrule 
  \end{tabular}
 \vspace{-10pt}
\end{table*}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/tables/tabular_benchmark.tex <==
\begin{table}[ht]
    \caption{F1-scores (in $\%$) and their standard deviations of 13 anomaly detection methods on tabular data. Results are taken from \citet{alvarez2022revealing}. The results indicate that NTL is the state-of-the-art for tabular anomaly detection.}
\label{tab:tab_benchmark}
 	\small
    \centering
  \begin{tabular}{l|ccccc|c}
  \toprule
     & KDDCUP10 & NSL-KDD & IDS2018& Arrhythmia & Thyroid & Avg.\\ 
  \midrule
ALAD & 95.9$\pm$0.7 & 92.1$\pm$1.5 & 59.0$\pm$0.0 & 57.4$\pm$0.4& 68.6$\pm$0.5 & 74.6  \\         
DAE & 93.2$\pm$2.0 &\bf96.1$\pm$0.1 &\bf71.5$\pm$0.5 & 61.5$\pm$2.5 & 59.0$\pm$1.5 & 76.3 \\
DAGMM & 95.9$\pm$1.4 &85.3$\pm$7.4 &55.8$\pm$5.3 & 50.6$\pm$4.7 & 48.6$\pm$8.0 & 67.2 \\
DeepSVDD &89.1$\pm$2.0 &89.3$\pm$2.0 &20.8$\pm$11 & 55.5$\pm$3.0&  13.1$\pm$13 & 53.6 \\
DROCC & 91.1$\pm$0.0 &90.4$\pm$0.0 &45.6$\pm$0.0 & 35.8$\pm$2.6 & 62.1$\pm$10 & 65.0 \\
DSEBM-e & 96.6$\pm$0.1 &94.6$\pm$0.1 &43.9$\pm$0.8 & 59.9$\pm$1.0 & 23.8$\pm$0.7 & 63.8 \\
DSEBM-r & \bf98.0$\pm$0.1 &95.5$\pm$0.1 &40.7$\pm$0.1 & 60.1$\pm$1.0 & 23.6$\pm$0.4 & 63.6 \\
DUAD & 96.5$\pm$1.0 &94.5$\pm$0.2 &\bf71.8$\pm$2.7 & 60.8$\pm$0.4 & 14.9$\pm$5.5 & 67.7 \\
MemAE &95.0$\pm$1.7 &95.6$\pm$0.0 &59.9$\pm$0.1 & 62.6$\pm$1.6& 56.1$\pm$0.9 & 73.8 \\
SOM-DAGMM &97.7$\pm$0.3 &95.6$\pm$0.3 &44.1$\pm$1.1 & 51.9$\pm$5.9 & 52.7$\pm$12 & 68.4 \\
LOF &95.1$\pm$0.0 &91.1$\pm$0.0 &63.8$\pm$0.0 & 61.5$\pm$0.0 & 68.6$\pm$0.0 & 76.0 \\
OC-SVM &96.7$\pm$0.0 &93.0$\pm$0.0 &45.4$\pm$0.0 & \bf63.5$\pm$0.0 & 68.1$\pm$0.0 &  73.3 \\
NTL &96.4$\pm$0.2 &\bf96.0$\pm$0.1 &59.5$\pm$8.9 & 60.7$\pm$3.7 & \bf73.4$\pm$0.6 & \bf77.2 \\
  \bottomrule 
  \end{tabular}
\end{table}

==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/thms/proof-thm2.tex <==
\begin{proof}
\vspace{-0.5em}
Let A1 and A2 denote Assumption 1 and 2, respectively. Furthermore, 
let $q(\vx_1, ..., \vx_{|\gQ|})$ and $q_s(s_1, ..., s_{|\gQ|})$ denote the query distribution in the data and anomaly score spaces, respectively. A2 assumes $\Ia_s(s):=\Ia_s(S(\vx))=\Ia(\vx)$ for all $\vx$. So the expectation of \Cref{eq:alpha-is} is 
\begin{align*}
&\E[\hat \alpha] = \E_{q(\vx_1, ..., \vx_{|Q|})}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(S(\vx_i))}{q_s(S(\vx_i))}\Ia(\vx)\right]  
\stackrel{A2}{=} \E_{q_s(s_1, ..., s_{|Q|})}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right] \\ 
& \stackrel{A1}{=} \E_{\prod_{i=1}^{|Q|}q_s(s_i)}\left[\frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|}\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right] 
= \frac{1}{|\gQ|}\sum_{i=1}^{|\gQ|} \E_{q_s(s_i)}\left[\frac{p_s(s_i)}{q_s(s_i)}\Ia_s(s_i)\right]
= \E_{p_s(s)}[\Ia_s(s)] \\
&= \E_{p(\vx)}[\Ia_s(S(\vx))]
\stackrel{A2}{=}\E_{p(\vx)}[\Ia(\vx)]=\alpha
\end{align*}
where the change of variables makes necessary assumptions, including the existence of density functions. \qedhere 


\vspace{-0.5em}
\end{proof}

















==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/thms/thm1-ranking.tex <==

\begin{theorem}
\label{thm:rank}
Let $\gQ_0$ be the index set of datapoints labeled normal and $\gQ_1$ the index set of datapoints labeled abnormal. 
Let $\delta \in \mathbb{R}^+$ be the smallest radius, such that for each unlabeled anomaly $\vu_a$ and each unlabeled normal datum $\vu_n$ there exist labeled data points $\vx_a, a\in\gQ_1$ and $\vx_n, n\in\gQ_0$, such that $\vu_a$ is within the $\delta$-ball of $\vx_a$ and $\vu_n$ is within the $\delta$-ball around  $\vx_n$. If a $\lambda_s$-Lipschitz continuous function $\s$ ranks the labeled data correctly, with a large enough margin, i.e. $\s(\vx_a)-\s(\vx_n) \geq 2\delta\lambda_s$,
then $\s$ ranks the unlabeled points correctly, too, and $\s(\vu_a)%
\geq\s(\vu_n)$.
\end{theorem}


==> hkcvkvkfkchjxcryzngnngtnvmcptrmw/thms/thm2-alpha.tex <==
\begin{theorem}
\label{thm:alpha}
Assume that Assumptions 1 and 2 hold. Then, \Cref{eq:alpha-is} is an unbiased estimator of the contamination ratio $\alpha$, i.e., $\E[\hat\alpha]=\alpha$.



\end{theorem}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
